Conformal model for gravitational waves and dark matter: A status update

We present an updated analysis of the first-order phase transition associated with symmetry breaking in the early Universe in a classically scale-invariant model extended with a new SU(2) gauge group. Including recent developments in understanding supercooled phase transitions, we compute all of its characteristics and significantly constrain the parameter space. We then predict gravitational wave spectra generated during this phase transition and by computing the signal-to-noise ratio we conclude that this model is well testable (and falsifiable) with LISA. We also provide predictions for the relic dark matter abundance. It is consistent with observations in a rather narrow part of the parameter space, since we exclude the so-called supercool dark matter scenario based on an improved description of percolation and reheating after the phase transition as well as inclusion of the running of couplings. Finally, we devote attention to renormalisation-scale dependence of the results. Even though our main results are obtained with the use of renormalisation-group improved effective potential, we also perform a fixed-scale analysis which proves that the dependence on the scale is not only qualitative but also quantitative.

==> sections/after-end-document.tex <==
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\section{Baryogenesis through leptogenesis}
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\begin{itemize}
\item ARS + Scalar decay mechanism, see~\cite{Hambye:2017, Hambye:2016}
\item Previous attempts in conformal models, see~\cite{Khoze:2013-2, Plascencia:2016, Hambye:2018}
\item ARS+scalar decays in another model: \cite{Baumholzer:2018}
\item Neutrino masses: \cite{Karam:2015}
\end{itemize}


%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\section{DM main results from previous analyses}
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

The $SU(2)_X$ dark matter model has been thoroughly studied in the literature. For the scale-invariant version see [REFs], while for the non-scale-invariant version see [REFs]. In this section, we collect the main results from these analyses.

\subsection{0811.0172 - Hidden vector dark matter
 (Hambye)}

\subsubsection{Relic density}

There is a number of tree level annihilation processes which determine the vector multiplet relic density through their freezeout. They can be classified in two classes. First the annihilations with no trilinear gauge interactions:
$A_i A_i \rightarrow \eta \eta, \,\eta h,\, h h$ via a direct quartic coupling or via an intermediate $h$ or $\eta$; and
$A_i A_i \rightarrow f \bar{f}, W^+ W^-, Z^0 Z^0$ via a $h$ or $\eta$ in the s-channel. Second the channels with one trilinear gauge coupling. These channels have the peculiar property (impossible with ordinary models based on a $Z_2$ symmetry) 
to involve one DM particle in the final state
by reducing the number of DM particles from 2 units to one unit.

\begin{figure}[h!]
\centering
\includegraphics[width=0.95\linewidth]{Annihdiag1.pdf}
\caption{\sf Annihilation diagrams with no DM particle in the final state} 
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[width=0.5\linewidth]{Annihdiag2.pdf}
\caption{\sf Annihilation diagrams with one DM particle in the final state} 
\end{figure}

\alex{The authors only took into account the annihilation cross sections, neglecting the semi-annihilations.}

\subsubsection{Direct detection}

At tree level a vector DM particle can collide elastically a nucleon either through $h$ exchange or via $\eta$ exchange, which results in a spin independent cross section
\begin{equation}
\sigma_{SI} (N A\rightarrow N A)=\frac{1}{64 \pi} f^2 g_\phi^4 \sin^2 2\beta \,m_N^2\frac{v_\phi^2}{v^2}  \frac{(m_\eta^2-m_h^2)^2}{m_\eta^4 m_h^4} \frac{m_r^2}{m^2_{A}} \,,
\label{directdetection}
\end{equation}
with $m_r=m_N m_{A}/(m_N+m_{A})$ the reduced mass and $m_N$ the nucleon mass. $f$ parametrizes the Higgs nucleon coupling, $f m_N \equiv \langle N | \sum_q m_q \bar{q}q|N\rangle=g_{hNN} v$. We take the value $f=0.3$.
For $m_{A}>>m_N$ numerically one gets:
\begin{equation}
\sigma (N A \rightarrow N A)=1.9 \cdot 10^{-44} \,\hbox{cm}^2 \cdot R\,\sin^2{2\beta}\,\Big(\frac{f}{0.3}\Big)^2 \Big(\frac{g_\phi}{0.5}\Big)^4 \Big( \frac{v_\phi}{500\,\hbox{GeV}}\Big)^2
 \Big(\frac{120\,\hbox{GeV}}{m_h}\Big)^4 \Big(\frac{100\,\hbox{GeV}}{m_A}\Big)^2
\end{equation}
with $R \equiv (m_\eta^2-m_h^2)^2/m_\eta^4$ which is unity for $m_\eta>>m_h$. This has to be compared with the present experimental upper bound on this cross section \cite{CDMS} which, for example around $m_{DM}=100$~GeV, is of order $10^{-44}$~cm$^2$. Therefore for not too small $\beta$ mixing angle the expected signal can be easily of order the present sensitivity or even exceed it by few orders of magnitude.

\subsubsection{Results}

\begin{figure}[h]
\begin{tabular}{c}
\includegraphics[width=7.3cm]{fig1a-6000points.png}
\includegraphics[width=7.3cm]{fig1b-6000points.png}
\end{tabular}
\caption{$g_\phi$ vs $v_\phi$ and $m_A$ vs $m_\eta$ leading to $0.091 \lesssim \Omega h^2 \lesssim 0.129$, for $10^{-7} < \lambda_m < 10^{-3}$, $m_h=120$~GeV and various values of $\lambda_\phi$: $\lambda_\phi= 10^{-4}$ (red), $\lambda_\phi= 10^{-3}$ (orange), $\lambda_\phi= 10^{-2}$ (green) and $\lambda_\phi= 10^{-1}$ (blue) (from left to right and top to bottom respectively). One also recognizes the $m_A =g_\phi v_\phi/2 \sim m_h/2$ resonant case curve.} \label{efficiencies}
\end{figure}

\begin{figure}[h]
\begin{tabular}{c}
\includegraphics[width=4.9cm]{fig2a-5500points.png}
\includegraphics[width=4.9cm]{fig2b-5500points.png}
\includegraphics[width=4.9cm]{fig2c-5500points.png}
%\includegraphics[width=5cm]{eta5sph11.eps}
\end{tabular}
\caption{For $10^{-3} < \lambda_m < 1$ and $114.4\,\hbox{GeV} < m_h < 180~\hbox{GeV}$, values of $g_\phi$ vs $v_\phi$, $m_A$ vs $m_\eta$ and $m_A$  vs $\sigma(AN \rightarrow A N)$ leading to $0.091 \lesssim \Omega h^2 \lesssim 0.129$.
$\lambda_\phi$ has been varied between $10^{-5}$ and $1$. 
Dots with $m_\eta\simeq 2 \, m_A$ proceed through resonance of the $\eta$ exchange diagrams (to $W^+W^-$, $ZZ$, $f \bar{f}$ or $hh$). Similarly dots with $m_h\simeq2 \, m_A$ similarly are dominated by the Higgs exchange diagrams (to $W^+W^-$, $ZZ$, $f \bar{f}$ or $\eta \eta$). Dots with   $m_\eta <114.4$~GeV are for suppressed values of $\sin \beta$ to agree with the LEP constraints on the $h \rightarrow f \bar{f}$ branching ratio.} 
\end{figure}

\subsection{0907.1007 - Confined hidden vector dark matter
 (Hambye \& Tytgat)}

\subsection{1306.2329 (CSI) - Dynamical generation of the weak and Dark Matter scale (Hambye \& Strumia)}

The DM thermal relic abundance and DM indirect signals require the computation of $\sigma v$, 
the non-relativistic DM annihilation cross section times the relative velocity $v$.
We compute them in the limit of small $\lambda_{HS}$, where  only 
$SU(2)_X$ gauge interactions are relevant,
and the mixing angle $\alpha$ is small, such that DM dominantly annihilates into $s$.
The model gives rise to $VV\to ss$  annihilations and to
$VV\to Vs$ semi-annihilations \cite{VDM} (see also \cite{VDM2,VDM3,othersemi}).
Averaging over initial spin and gauge components we find:
\beq \sigma v_{\rm ann} =\frac{11g_X^2}{1728\pi w^2}
%\frac{43}{3456\pi} \frac{g_X^2}{w^2}
,\qquad
\sigma v_{\rm semi-ann} = \frac{g_X^2}{32\pi w^2}.
\eeq
The cosmological DM abundance is reproduced as a thermal relic for
$\sigma v_{\rm ann}+ \frac{1}{2}\sigma v_{\rm semi-ann}\approx 2.2~10^{-26}\,{\rm cm}^3/{\rm s}$, which means
\begin{equation}
g_X \simeq w/2.0\TeV .
\end{equation}
%\footnote{The result agrees with the numerical results of \cite{VDM3},
%in the limit where no resonant scatterings happens, as predicted by the present model.}

\bigskip

With this assumption, the model only has one free parameter:
out of the 4 parameters $\lambda,\lambda_{HS}, \lambda_S$ (or $s_*$) and $g_X$,
3 of them are fixed by the observed Higgs mass and vacuum expectation value, and by the cosmological DM abundance $\Omega_{\rm DM}$~\cite{Planck}.
We can view $g_X$ or $\lambda_{HS}$ as the only free parameter.
They are related as
\beq \lambda_{HS} \simeq 0.004/g_X^2\label{eq:rel}\eeq
The observables are predicted in terms of $g_X$ as
%\begin{eqnsystem}{sys:pars}
%m_2 &\simeq& 165\GeV (\lambda_{HS}/0.004)^{-3/2},\qquad\\
%\alpha &\simeq& 0.07 (\lambda_{HS}/0.004)^{7/2},\\
%g_X &\simeq& 1.00 (\lambda_{HS}/0.004)^{-1/2}, \\
%M_X &\simeq&  985\GeV (\lambda_{HS}/0.004)^{-1} ,\\
%\sigma_{\rm SI} 
%%\stackrel{m_1\ll m_2}{\sim}
%&\simeq& 0.7~10^{-45}\,{\rm cm}^2\, (\lambda_{HS}/0.004)^6 \Big[1-(m_1^2/m_2^2)\Big]^2.
%\end{eqnsystem}
\beq
\begin{array}{rclrcl}
m_2 &\simeq& 165\GeV g_X^3,\qquad \qquad&
\alpha &\simeq& 0.07/g_X^7,\\
M_X &\simeq&  985\GeV g_X^2,&
\sigma_{\rm SI} 
%\stackrel{m_1\ll m_2}{\sim}
&\simeq& 0.7~10^{-45}\,{\rm cm}^2\, \Big[1-(m_1^2/m_2^2)\Big]^2/g_X^{12} .
\end{array}\eeq
where $\sigma_{\rm SI}$ is the DM direct detection cross section, computed below.
These approximations hold in the limit of small $\lambda_{HS}$, which numerically means
$\lambda_{HS}\ll \sqrt{\lambda_H\lambda_S}\approx 0.015$ i.e.\ $g_X \gg 0.5$.
%When approximating $\sigma_{\rm SI}$ we also assumed $m_1\ll m_2$.
Fig.\fig{FS} shows the same predictions, computed numerically without making the small $\lambda_{HS}$ approximation.

\medskip


\begin{figure}[t]
\begin{center}
$$\includegraphics[height=7cm]{figH}\qquad
\includegraphics[height=7cm]{figDM}$$
\caption{\em   Predicted cross sections for the extra scalar boson  (left) and for DM direct detection  (right) as function of 
the only free parameter of the model $\lambda_{HS}$, varied as shown in the colour legend.
%Future experiments should be able of improving the sensitivity to the extra Higgs cross section 
%by $1-2$ orders of magnitudes 
%and the sensitivity to $\sigma_{\rm SI}$ by $2-3$ orders of magnitude before 2020.
\label{fig:FS}}
\end{center}
\end{figure}

The Spin-Independent cross section for DM direct detection is~\cite{VDM}
%\beq \sigma_{\rm SI} = \frac{g_X^4 f^2 }{64\pi}\frac{w^2}{v^2}\frac{m_N^4 }{M_X^2}
%\sin^2 2\alpha \bigg(\frac{1}{m_1^2} - \frac{1}{m_2^2}\bigg)^2
%\eeq
\beq \sigma_{\rm SI} = \frac{m_N^4  f^2 }{16\pi v^2}
 \bigg(\frac{1}{m_1^2} - \frac{1}{m_2^2}\bigg)^2 g_X^2 \sin^2 2\alpha
\eeq
where $f\approx 0.295$ is the nucleon matrix element and $m_N$ is the nucleon mass.
Fig.\fig{FS}b shows the predictions for DM direct searches.  Present direct detection constraints imply
the bounds $\lambda_{HS}\lesssim 0.007$ (so that the 
approximation of small $\lambda_{HS}$ holds in the  
phenomenologically interesting region), $m_2\gtrsim 70$~GeV, $w\gtrsim1.5$~TeV, 
$M_X\gtrsim  560\GeV$,
$g_X\gtrsim 0.75$ and $\alpha\lesssim 0.5$. 
A value of $\lambda_{HS}=0.007$ is also disfavoured by LEP Higgs searches (fig.\fig{FS}a).

\subsection{1307.8428 (CSI) - Classical scale-invariance, the electroweak scale and vector dark matter (Carone \& Ramos)}

\begin{figure}[H]
    \includegraphics[width=0.495\textwidth]{allowed3p.pdf} 
    \caption{Band where the dark gauge multiplet provides the dark matter relic density within $\pm2\sigma$ experimental
    uncertainty.}  
    \label{fig:relicallowed}
\end{figure}

``we omit diagrams that change dark matter number by only one unit, i.e., 
$AA\to A\eta$"

We find that the thermally averaged annihilation cross section times relative velocity is
\begin{align}
 \langle\sigma_{\text{ann}} v\rangle=&\frac{g_D^4 \cos^4\theta}{192\pi m_A^2}\sqrt{1-\frac{m_\eta^2}{m_A^2}}\left[\left
 (\frac{3}{2}\frac{\lambda \langle\varphi\rangle^2\cos^2\theta }{\left(4m_A^2-m_\eta^2\right)}+\frac{1}{2}\right)^2\right.
 \nonumber\\
 &\left.-\frac{4}{3} \left(\frac{m_A^2}{m_\eta^2-2 m_A^2}\right)^2 \left(8-6\frac{m_\eta^2}{m_A^2}+\frac{m_\eta^4}
 {m_A^4}\right) \left(\frac{3}{2}\frac{\lambda \langle\varphi\rangle^2\cos^2\theta}{\left(4
   m_A^2-m_\eta^2\right)}+\frac{1}{2}\right)\right.\nonumber\\
   &\left.+\frac{4}{3}\left(\frac{m_A^2}{m_\eta^2-2 m_A^2}\right)^2 \left(6-4\frac{m_\eta^2}{m_A^2}
   +\frac{m_\eta^4}{m_A^4}\right)\right].
\end{align}
From this result, the freeze-out temperature and relic density are numerically calculated. With $x \equiv m_A/T$,
we find numerically that the freeze-out temperature is typically in the range $x_F \approx 26 - 27$.   The relic
density is given by
\begin{equation}
\Omega_D h^2 \approx 3 \cdot \frac{(1.07 \times 10^9 \mbox{ GeV}^{-1}) \, x_F}
{\sqrt{g_*(x_F)} M_{Pl} \langle \sigma v \rangle_F}
\end{equation}
where the factor of $3$ takes into account the size of the SU(2)$_D$ gauge multiplet.    As a point of reference,
we note that if all species are dynamical and in equilibrium, one would find $g_*=122$.

The dark matter-nucleon 
elastic scattering cross section is given by
\begin{equation}
\sigma(NA\to NA)=\frac{1}{64\pi}f^2g_D^4\sin^2 2\theta \frac{m_N^2}{m_A^2}\frac{\langle\varphi\rangle^2}{\langle\sigma\rangle^2}\frac{(m_\eta^2-m_h^2)^2}{m_\eta^4m_h^4}\left(\frac{m_Nm_A}{m_N+m_A}\right)^2
\label{eq:ddsig}
\end{equation}
where $m_N$ is the nucleon mass and $f$ parameterizes the Higgs-nucleon coupling.

\subsection{1403.4953 (CSI) - Higgs vacuum stability from the dark matter portal (Khoze, McCabe \& Ro)}

Having argued that the vector triplet and scalar particles are stable and therefore potential dark matter candidates, we must calculate the relic abundance in order to show that they can saturate, or form a component of the observed dark matter abundance, for which we take $\Omega_{\rm{DM}} h^2=0.1187\pm0.0017$, the value inferred from Planck+WP+HighL+BAO data~\cite{Ade:2013zuv}. Owing to the reasonable couplings to the Standard Model particles, the scalar and vector dark matter components
are in thermal equilibrium with the Standard Model degrees of freedom in the early Universe. Their abundance is therefore determined by the thermal freeze-out mechanism. To calculate it, we must solve the Boltzmann equation, which is~\cite{Gondolo:1990dk, D'Eramo:2010ep},
\begin{equation}
\frac{d n_i}{dt}+3Hn_i=-\langle\sigma_{ii}v\rangle\left(n_i^2-n_i^{\rm{eq}\,2} \right)-\sum_{j,k}\langle\sigma_{ijk}v\rangle\left(n_i n_j-\frac{n_k}{n_k^{\rm{eq}}}n_i^{\rm{eq}}n_j^{\rm{eq}}\right)\;,
\end{equation}
where $n_i$ is the number density of one component $\chi_i$ of the dark matter abundance, $\langle\sigma_{ii}v\rangle$ is the usual annihilation cross-section term for reactions of the form $\chi_i \chi_j\to X X$, where $X$ is a particle in equilibrium with the thermal bath,
 and $\langle\sigma_{ijk}v\rangle$ is the cross-section for the semi-annihilation reaction $\chi_i \chi_j\to \chi_k X$.
 
 \begin{figure}[t!]
\centering
\includegraphics[width=0.99 \columnwidth]{semiann2.pdf}
\includegraphics[width=0.99 \columnwidth]{ann2.pdf}
\caption{
The upper three diagrams show the process $Z'_i Z'_j\to Z'_k h_2$, which is the dominant contribution to the semi-annihilation cross-section. The process $Z'_i Z'_j\to Z'_k h_1$ also occurs but is suppressed by $\tan^2\theta$.  The lower four diagrams show the processes that dominate the annihilation of $Z'_i Z'_i$. Other diagrams are suppressed by at least one power of $\sin\theta$ or $\lambda_{\rm{P}}$.}
\label{fig:semiann}
\end{figure}

We first consider the case of vector dark matter only, which is similar to Hambye's model~\cite{Hambye:2008bq} except that here there are no explicit $\mu$ terms. This model is interesting as it was the first example of a model containing both annihilation and semi-annihilation processes, as shown in fig.~\ref{fig:semiann}. 

The annihilation cross-section is dominated by the lower four diagrams of fig.~\ref{fig:semiann}, which contribute to the process $Z^{'}_i Z^{'}_i \to h_2 h_2$. The leading order terms contributing to the non-relativistic (s-wave) cross-section from these diagrams are 
\begin{equation}
\label{eq:xsecij}
\langle\sigma_{ii} v\rangle=\frac{11g_{\sst \mathrm{CW}}^4-60 g_{\sst \mathrm{CW}}^2 \lambda_{\phi}+108 \lambda_{\phi}^2}{2304\pi}\,\frac{ \cos^4\theta}{ M^2_{Z'}}+\mathcal{O}\left(\frac{m^2_{h_2}}{M^2_{Z'}},\sin\theta,\lambda_{\rm{P}}\right)\;.
\end{equation}
In our numerical work, we include all sub-leading terms in this cross-section as well as including the contributions from $Z'_i Z'_i\to h_1 h_1$, $Z'_i Z'_i\to\bar{f}f$, $Z'_i Z'_i\to W^{+}W^{-}$ and $Z'_i Z'_i\to Z^{0}Z^{0}$, all of which are suppressed by at least one power of $\sin\theta$ or $\lambda_{\rm{P}}.$

The diagrams that contribute to the semi-annihilation process are shown by the upper three diagrams in fig.~\ref{fig:semiann}. In the non-relativistic limit, the (s-wave) cross-section for $Z'_i Z'_j\to Z'_k h_2$ is
\begin{equation}
\label{eg:xsecijk}
\langle\sigma_{ijk} v\rangle=\frac{3 g_{\sst \mathrm{CW}}^4}{128 \pi}\frac{\cos^2\theta}{ M_{Z'}^2}\left(1-\frac{m_{h_2}^2}{3 M_{Z'}^2}\right)^{-2}\left(1-\frac{10 m_{h_2}^2}{9 M_{Z'}^2} +\frac{m_{h_2}^4}{9 M_{Z'}^4}\right)^{3/2}\;.
\end{equation}
There is also a subdominant process $Z'_i Z'_j\to Z'_k h_1$ whose cross-section is obtained from eq.~\eqref{eg:xsecijk} by substituting $m_{h_2}\to m_{h_1}$ and $\cos\theta\to\sin\theta$. For completeness, we include this in our numerical work. Comparing eqs.~\eqref{eq:xsecij} and \eqref{eg:xsecijk}, we observe that $\langle\sigma_{ijk} v\rangle\sim5\langle\sigma_{ij} v\rangle$ so the semi-annihilation processes dominate.

The global custodial symmetry ensures that the vector triplet is degenerate in mass and each $Z'_i$ contributes one-third to the relic abundance. That is the total abundance $n_{Z'}$ is related to the individual components by $n_{Z'}=3 n_{Z'_1}=3 n_{Z'_2}=3 n_{Z'_3}.$
It should also be clear that $\langle\sigma_{11}v\rangle=\langle\sigma_{22}v\rangle=\langle\sigma_{33}v\rangle:=\langle\sigma v\rangle_{\rm{ann}}$ and $\langle\sigma_{123}v\rangle=\langle\sigma_{132}v\rangle=\langle\sigma_{213}v\rangle=\langle\sigma_{231}v\rangle=\langle\sigma_{312}v\rangle=\langle\sigma_{321}v\rangle:=\langle\sigma v\rangle_{\rm{semi-ann}}$. Therefore, the Boltzmann equation for the total abundance is
\begin{equation}
\label{eq:Boltzvect}
\frac{d n_{Z'}}{dt}+3H n_{Z'}=-\frac{\langle\sigma v\rangle_{\rm{ann}}}{3}\left(n_{Z'}^2-n_{Z'}^{\rm{eq}\,2} \right)-\frac{2\langle\sigma v\rangle_{\rm{semi-ann}}}{3}n_{Z'}\left(n_{Z'} - n_{Z'}^{\rm{eq}}\right)\;.
\end{equation}
We solve this equation numerically by the method outlined in~\cite{Belanger:2012vp}.

\begin{figure}[t!]
\centering
\includegraphics[width=0.49\columnwidth]{su2_dm.pdf}\hspace{2mm}\includegraphics[width=0.49 \columnwidth]{su2_dm_ma_mh2.pdf}
\caption{
The coloured contours and the wedge-shaped regions in black in both panels indicate when the vector triplet forms more less than 100\%, 10\% and 1\% of the observed dark matter abundance, and the parameter values where the Higgs potential is stabilised respectively. Also shown in the left panel are the LUX and projected LZ limits (the region above these lines is excluded), which account for the fact that the dark matter is a subcomponent of the total density in much of the parameter space, and the limit $\sin^2\theta=0.1$. The right panel shows that the vector mass should lie between 500~GeV and 1~TeV to improve Higgs stability.}
\label{fig:vector_relic}
\end{figure}


The coloured regions in the left and right panels of fig.~\ref{fig:vector_relic} show the total relic abundance of the vector triplet as a fraction of the observed abundance. For instance, in the lower left  (blue) part of the left panel, the abundance exceeds the observed value and is therefore excluded. The thick black wedge indicates the region where the Higgs potential is stabilised up to the Planck scale (as in fig.~\ref{SU2Stab}). We see that for most of wedge, the vector triplet contributes between 1\% and 100\% of the total dark matter abundance. 
However, when we combine this with the LHC constraint on $\sin^2 \theta$, we see from fig.~\ref{fig:vector_relic} that the vector
dark matter component contributes less than 10\% to the total relic abundance, and we need to add another dark matter component.
The right panel in fig.~\ref{fig:vector_relic} shows the dark matter fraction as a function of $M_{Z'}$ and $m_{h_2}$. To lie within the
Higgs vacuum stability wedge, we see that the $M_{Z'}$ lies between 500~GeV and 1000~GeV.

Also shown on the left panel are the direct detection current constraints from LUX~\cite{Akerib:2013tjd} and the projected limits from LZ~\cite{Cushman:2013zza}. At a direct detection experiment, a vector $Z'_i$ can elastically scatter with a nucleon $N$ via exchange of $h_1$ or $h_2$. The resulting spin-independent scattering cross-section for this to occur is
\begin{equation}
\sigma_{N}^{\rm{SI}}=\frac{g_{\sst \mathrm{CW}}^2 \sin^2 2\theta }{16 \pi}\frac{f_N^2 m_{N}^2 \mu_{\rm{red}}^2}{v^2}\left(\frac{1}{m_{h_2}^2}-\frac{1}{m_{h_1}^2} \right)^2\;,
\end{equation}
where $f_N:=\bra{N}\sum_q m_q \bar{q}q \ket{N}/m_N \approx 0.295$ is the Higgs-nucleon coupling~\cite{Cheng:2012qr}, $m_N$ is the nucleon mass and $\mu_{\rm{red}}$ is the vector-nucleon reduced mass. When setting a limit from the experimental data, we account for the fact that the the vector triplet forms a subcomponent of the total dark matter density over much of the parameter space of interest. We make a scaling ansatz that the fraction of the local dark matter density $\rho_{Z'}/\rho_{\rm{DM}}$ is the same as the fraction of the dark matter relic abundance $\Omega_{Z'}/\Omega_{\rm{DM}}$. The limits from LUX and LZ after taking into account this scaling are shown in fig.~\ref{fig:vector_relic} by the lines with the appropriate label. In the left panel, the region above and to the left of the lines are excluded. 
We have also checked that the LUX exclusion limit, when applied to the right panel, excludes the entire lower island. 
Therefore, while the current LUX limits do not constrain the region where the Higgs potential is stabilised, the projected LZ limit excludes all of this region.

\subsection{1404.4977 - A weighty interpretation of the Galactic Centre excess (Boehm, Dolan \& McCabe)}

\begin{figure}[H]
 \centering
 \includegraphics[width=1.0\columnwidth]{semiann3.pdf}\\ \vspace{1mm}
 \includegraphics[width=1.0 \columnwidth]{ann3.pdf}
 \caption{
 A subset of the diagrams contributing to the production of on-shell $\eta$ particles from semi-annihilation (upper diagrams) and annihilation (lower diagrams) of the DM $Z'^{a}$. The diffuse $\gamma$ spectrum arises from the decay products of $\eta\to f\bar{f}$. The direct annihilation to Standard Model particles is suppressed by $\sin^2\theta\lesssim 10^{-4}$. }
 \label{fig:Feyn}
 \end{figure}
 
 The trilinear gauge coupling allows for semi-annihilation processes $Z'^{a} Z'^{b}\to Z'^{c} \eta$ represented in fig.~\ref{fig:Feyn}. The corresponding cross-section is given by
 \begin{equation}
 \label{eg:xsecijk}
 \langle\sigma v\rangle_{\rm{semi}}=\frac{ \gD^4 \cos^2\theta}{128 \pi M_{Z'}^4}\frac{\left( 9 M_{Z'}^4-10m_{\eta}^2 M^2_{Z'}+m^4_{\eta} \right)^{3/2}}{\left(m^2_{\eta}-3 M^2_{Z'} \right)^2}.
 \end{equation}
 We do not include semi-annihilation into $h_{\rm{SM}}$ as it is kinematically forbidden for $M_{Z'}< m_{h_{\rm{SM}}}$.

The dominant annihilation channel corresponds to $Z'^{a}Z'^{a}\to \eta \eta$ and is illustrated in fig.~\ref{fig:Feyn}. The analytic expression for the corresponding cross-section ($\langle\sigma v \rangle_{\rm{ann}}$) is lengthy so we do not give it here. However, in fig.~\ref{fig:ratio}, we show the ratio $\langle\sigma v\rangle_{\rm{semi}}/\langle\sigma v \rangle_{\rm{ann}}$ for $\sin\theta=10^{-2}$ and various ratios of $m_{\eta}/M_{Z'}$.

In this plot we include all possible final states when they are kinematically accessible, including the direct $2 \to 2$ process with $Z'^{a}Z'^{a}\to \bar{f}f,W^{+}W^{-},Z^{0}Z^{0}$, even though they are suppressed by $\sin^2\theta$ (constraints discussed later require $\sin\theta\lesssim10^{-2}$). This suppression arises because $Z'^{a}$ and $\eta$ are only connected to the SM sector through $\lambdaP\propto\sin\theta$. We observe that in that regime the semi-annihilation process dominates unless $m_{\eta}\approx M_{Z'}$; annihilation eventually dominates because the phase-space suppression is faster for the semi-annihilation process. An exception is at $2M_{Z'}\approx \mhSM$ where $\langle\sigma v \rangle_{\rm{ann}}$ becomes resonantly enhanced through the diagram shown in the bottom left of fig.~\ref{fig:Feyn}. The results in fig.~\ref{fig:ratio} are unchanged for smaller values of $\sin\theta$ and furthermore, are to a very good approximation independent of $\gD$. This is because $\lambda_{\phi}\approx \gD^2 m^2_{\eta}/2 M_{Z'}^2$ for $\sin\theta \lesssim10^{-2}$, with the result that both the semi-annihilation and annihilation cross-sections scale as $\gD^4$ so the dependence of $\langle\sigma v\rangle_{\rm{semi}}/\langle\sigma v \rangle_{\rm{ann}}$ on $\gD$ drops out.

 \begin{figure}[H]
 \centering
 \includegraphics[width=0.943\columnwidth]{ratio.pdf}
 \caption{
 Ratio of the semi-annihilation to annihilation cross-section. We have fixed $\sin\theta=10^{-2}$ and the ratio $m_{\eta}/M_{Z'}$ to the values specified in the plot. Semi-annihilation dominates when $m_{\eta}< M_{Z'}$; annihilation dominates when $m_{\eta} \approx M_{Z'}$.
 }
 \label{fig:ratio}
 \end{figure}

\subsection{1406.4104 (CSI) - Predictions of a model of weak scale from dynamical breaking of scale invariance (Pelaggi)}

\subsection{1505.07480 - Non-Abelian gauge fields as dark matter (Gross, Lebedev \& Mambrini)}

\begin{figure}[H] 
\centering{
\includegraphics[scale=0.43]{U1ST03MHp280DM1TeV.pdf}
\includegraphics[scale=0.43]{U1ST03MHp1000DM2TeV.pdf}
\includegraphics[scale=0.43]{U1ST02MHp3000DM3TeV.pdf}
\includegraphics[scale=0.43]{SU2ST03MHp280DM1TeV.pdf}
\includegraphics[scale=0.43]{SU2ST03MHp1000DM2TeV.pdf}
\includegraphics[scale=0.43]{SU2ST02MHp3000DM3TeV.pdf}
}
\caption{ \label{plots}
Constraints on the gauge coupling $\tilde g$ vs DM mass $m_A$ for U(1) and SU(2).
The area between the red lines is favoured by the DM relic abundance, while the regions above 
the dashed blue, dotted black and green lines are ruled out by direct detection, indirect detection and perturbativity of $\lambda_i$, respectively.
{\it Upper row:} U(1) dark matter with $\sin\theta=0.3, m_{h_2}= 280$ GeV (left),
 $\sin\theta=0.3, m_{h_2}= 1$ TeV (center), $\sin\theta=0.2, m_{h_2}= 3$ TeV (right).
 {\it Lower row:} SU(2) dark matter with $\sin\theta=0.3, m_{h_2}= 280$ GeV (left),
 $\sin\theta=0.3, m_{h_2}= 1$ TeV (center), $\sin\theta=0.2, m_{h_2}= 3$ TeV (right). 
}
\end{figure}

Aside from the gauge self--interactions, the Lagrangian (\ref{DMinteractions}) applies
to the SU(2) case as well, up to the summation over the 3 species, $A_\mu A^\mu 
\rightarrow A_\mu^a A^{a \mu }$. The main change compared to the U(1) case is that 
the annihilation cross section decreases since only the species with the same group index 
can annihilate through the Higgs--like states. In order to keep the same relic abundance, one needs to increase the gauge coupling. Since the $s$--channel annihilation through $h_{1,2}$
often dominates, this amounts approximately to
\begin{equation}
\tilde g \rightarrow \sqrt{3} \tilde g \;,
\end{equation}
whereas if 
 the $t$--channel and the quartic interactions dominate, the rescaling factor is closer
 to $3^{1/4}$. The direct detection constraint remains the same as in the U(1) case since particles with different group indices scatter the same way on nucleons.
This decreases somewhat the allowed parameter space compared to the Abelian case (Fig.~\ref{plots}).

Non--Abelian DM features a semi--annihilation channel $AA \rightarrow A h_{1,2}$
(Fig.~\ref{diagrams2}).
In some regimes, for example at large $\tilde g$ and small $\sin\theta$, it can even dominate~\cite{D'Eramo:2012rr} (see also~\cite{Arina:2009uq,Khoze:2014xha}). 
Using the analytical results of~\cite{D'Eramo:2012rr},
we find that DM semi--annihilation is insignificant in the relevant parameter regions.
For example, at $m_A > m_{h_2}$ the $\sin\theta$--unsuppressed and potentially important channel $AA \rightarrow A h_2$ opens up, yet it is dominated by $AA \rightarrow h_2 h_2$.
Also, around the resonances the gauge coupling is rather small which diminishes the relative importance of semi--annihilation. 

No firm conclusion can be reached as to whether the region $m_A > m_{h_2}$ is allowed.
As stated above, the uncertainties in $f_N$ play a critical role due to the proximity of the Planck band and the LUX bound.

\subsection{1506.03285 (CSI) - A minimal model for SU(N) vector dark matter (Di Chiara \& Tuominen)}

As we pointed out in the previous subsection, the residual SO$(N)$ makes the massive $A^a$ vector bosons stable and therefore suitable dark matter candidates. Their annihilation and semi-annihilation cross sections can be easily calculated in the limit of zero portal coupling $\lambda_p$. This approximation for the dark matter analysis is consistent, as in the next section it turns out that $\lambda_p\ll g_D$ in the viable region of parameter space. 

For the thermally averaged annihilation ($AA\rightarrow \sigma\sigma$) and semi-annihilation ($AA\rightarrow \sigma A$) cross section times relative velocity we find
\be
\langle \sigma v\rangle_{\rm{ann}} =\frac{11 m_A^2}{144 \left(N^2-1\right) \pi  v_{\phi }^4}\ ,\quad \langle \sigma v\rangle_{\rm{semi-ann}} =\frac{3 m_A^2}{8 \left(N^2-1\right) \pi  v_{\phi }^4}\ ,
\ee
which for $N=2$ reproduce the results of \cite{Hambye:2013dgv,Carone:2013wla}. This approximation is sufficient when working away from the resonance thresholds, where the full thermal average \cite{Gondolo:1990dk} should be used; see e.g. \cite{Cline:2013gha}.

The dark matter abundance is determined by 
\be
\frac{dY}{dx}=Z(x)\left(\langle \sigma v\rangle_{\rm{ann}} (Y^2-Y_{\rm{eq}}^2)+\frac{1}{2}\langle \sigma v\rangle_{\rm{semi-ann}} Y(Y-Y_{\rm{eq}})\rangle\right),
\ee
where $Y=n/s$, $Y_{\rm{eq}}$ the corresponding equilibrium density, $x=m_A/T$, and 
\be
Z(x)=-\sqrt{\frac{\pi}{45}}M_{\rm{Pl}} m_A\sqrt{g_\ast(m_A/x)}x^{-2} \ ,
\ee
with $g_*$ denoting the effective number of degrees of freedom and $M_{Pl}$ the Planck mass. 

Using the standard approximations, the dark matter abundance is determined by
\be\label{Ohs}
\Omega h^2=N\frac{1.07\times 10^9 {\rm GeV}^{-1} x_f}{\sqrt{g_*\left(x_f\right)}M_{\rm{Pl}}\langle v\sigma \rangle}\ ,\quad \langle \sigma v\rangle=\langle \sigma v \rangle_{\rm{ann}}+\frac{1}{2}
\langle \sigma v\rangle_{\rm{semi-ann}} \ .
\ee
The value of $x_f=m_A/T_f$ is determined by solving 
 \be
 x_f=\ln\left[\frac{Z(x_f)y_{\rm{eq}}(x_f)^2}{y^\prime_{\rm{eq}}(x_f)-y_{\rm{eq}}(x_f)}\left(\frac{\delta(\delta+2)}{\delta+1}\langle \sigma v\rangle_{\rm{ann}}+\frac{\delta}{2}\langle \sigma v\rangle_{\rm{semi-ann}}\right)\right],
 \ee
where $\delta$ determines the deviation of the distribution from the equilibrium one, $\delta=Y/Y_{\rm{eq}}-1$, before the freeze out. The value of $\delta$ is expected to be ${\cal{O}}(1)$, and in the numerical analysis we choose $\delta=1$.

\begin{figure}[H]
\centering
\includegraphics[width=0.46\textwidth]{gDlp2b.png}\hspace{1cm}
\includegraphics[width=0.46\textwidth]{gDlp3.png}\hspace{0.1cm}
\caption{Portal coupling as a function of the dark gauge coupling for $N=2$ (left panel) and $N=3$ (right panel) in color for stable and perturbative data points, with color code function of $c_\alpha=\cos\alpha$ as given by the bar in the left panel. The data points that also produce an experimentally viable dark matter abundance are shown in black, and the gray points represent the unstable and/or non-perturbative data points which though feature a viable coupling coefficient $c_\alpha$.}
\label{gDlp}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=0.46\textwidth]{mDmp2b.png}\hspace{1cm}
\includegraphics[width=0.46\textwidth]{mDmp3.png}\hspace{0.1cm}
\caption{Dark scalar and dark vector masses for all the data points satisfying the LHC constraint, for $N=2$ (left panel) and $N=3$ (right panel), in color for those that also feature stability and perturbativity, in black those that satisfy the dark matter abundance constraint as well, while the data points that do not satisfy neither of the last two constraints are in gray.}
\label{mDmp}
\end{figure}

We compare the numerical result produced by Eq.~\eqref{Ohs} at each viable data point with the 95\% experimental interval \cite{Ade:2015xua}
\be\label{DMrd}
\Omega h^2=0.1193\pm0.0028\ ,
\ee
and find 23 data points (or 1\% of the total) for $N=2$ (Figs.~\ref{gDlp},\ref{mDmp}, left panels) and 39 (or 2\% of the total) for $N=3$ (Figs.~\ref{gDlp},\ref{mDmp}, right panels) that satisfy the dark matter constraint above as well as those in Eqs.~(\ref{LHCc},\ref{pstabc}).

Finally, we also impose the direct detection constraints. The spin independent cross section for the elastic scattering off a nucleon  $\cal N$ of the vector dark matter candidate, $A^a$, mediated by either $h_1$ or $h_2$ is, in the limit $m_A\gg m_{\cal N}$,
\be\label{sSI}
\sigma_{SI}\left({\cal N} A\rightarrow {\cal N} A\right)=\frac{f_{\cal N}^2 m_{\cal N}^4 m_A^2}{64 \pi  v_h^2 v_{\phi }^2} \sin^2 2 \alpha \left(\frac{1}{m_1^2}-\frac{1}{m_2^2}\right)^2\ ,
\ee
where $f_{\cal N}=0.303$ is the effective Higgs nucleon coupling \cite{Cline:2013gha}\footnote{We thank K. Kainulainen for discussions on this and for providing an updated value}, $m_{\cal N}=0.939$ GeV is the average nucleon mass. 
In the mass range of interest to us here, $m_D\sim{\cal O}(100)$ GeV, the most stringent bounds are provided by the LUX experiment \cite{Akerib:2013tjd}. We evaluate Eq.~\eqref{sSI} at each data point and compare with the experimental constraint in \cite{Akerib:2013tjd}, as a function of the mass of the dark matter candidate, $m_A$: all the data points satisfying the LHC constraint on the Higgs couplings, Eq.~\eqref{LHCc}, and consequentially also the points satisfying the stability, perturbativity, and dark matter abundance constraints, are viable. In more detail we obtain that the experimental constraint on the spin independent cross section is on average an order of magnitude larger than the predicted value
\be
N=\left\{\begin{array}{c}
2\\ 3
\end{array}\right.
\ , \quad
\sigma_{SI}\left({\cal N} A\rightarrow {\cal N} A\right)=\begin{array}{c}
(5\pm 4)\times 10^{-46}~ {\rm cm^2}\\ (3\pm 3)\times 10^{-46}~ {\rm cm^2}
\end{array}\ .
\ee

\subsection{1510.08063 - Production Regimes for Self-Interacting Dark Matter (Bernal, Carcia-Cely, Hambye et al.)}

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.3\textwidth]{gd1.pdf}
\includegraphics[width=0.3\textwidth]{gd2.pdf}
\includegraphics[width=0.3\textwidth]{gd3.pdf}\\
\includegraphics[width=0.3\textwidth]{gd4.pdf}
\includegraphics[width=0.3\textwidth]{gd5.pdf}
\end{center}
\caption{ \textit{Diagrams for dark matter self-interactions.}
}
\label{fig:selfDM}
\end{figure}

\begin{figure}[ht!]
\centering
\includegraphics[width=0.3\textwidth]{d1.pdf}
\includegraphics[width=0.3\textwidth]{d2.pdf}
\includegraphics[width=0.3\textwidth]{d3.pdf}\\
\includegraphics[width=0.3\textwidth]{d4.pdf}
\includegraphics[width=0.3\textwidth]{d5.pdf}
\includegraphics[width=0.3\textwidth]{d6.pdf}\\
\includegraphics[width=0.3\textwidth]{d7.pdf}
\includegraphics[width=0.3\textwidth]{d8.pdf}
\includegraphics[width=0.3\textwidth]{d9.pdf}\\
\includegraphics[width=0.3\textwidth]{d10.pdf}
\includegraphics[width=0.3\textwidth]{d11.pdf}
\caption{ \textit{Tree level diagrams for the process $AA\leftrightarrow AAA$.}
}
\label{xx-xxx}
\end{figure}

There are many physical mechanisms that can lead to self-interacting DM. In the HVDM model, this arises in two different ways: via the exchange of the scalar mediators $\eta$ or $h$ (Fig.~\ref{fig:selfDM}-bottom) or via the quartic and cubic hidden gauge interactions (Fig.~\ref{fig:selfDM}-top). If the mediators are heavier than the DM, the latter processes typically dominate. In this case 
the perturbative calculation is reliable and the corresponding cross section depends only mildly on the non-relativistic DM velocity. In particular, in the limit of small mixing and vanishing relative velocity, the Born approximation cross section reads 
%
\begin{equation}
\label{sigmaAAAApert}
\sigma_{AA}=\frac{65}{9}\,\frac{\alpha_X^2}{\ma^2} \left[1+ {\cal O}\left(\frac{\ma^2}{\meta^2} \right)\right]\,.
\end{equation}
%
Of particular importance is the fact that in this case, if $\alpha_X\lesssim 1$, in order to obtain the order of magnitude associated to the solution of small-scale problems, i.e. $\sigma_{AA}/\ma\sim 0.1$~cm$^2$/g, one needs $\ma \lesssim 400$\,MeV. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.49\textwidth]{ma-alpha2.pdf} 
\includegraphics[width=0.49\textwidth]{ma-som2.pdf} 
\caption{ Values of $\alpha_X$ and $m_A$ which yield the observed DM relic density. The black solid lines correspond to thermal production of DM via the 3-to-2 mechanism under the assumption of kinetic  equilibrium (i.e.~$T=T'$) until freeze-out. 
The gray, red and blue lines  give a value of $\sigma_{AA}/\ma$ equal to 0.1, 1 and 10 cm$^2/$g, respectively.
The area where perturbation theory breaks down, $\alpha_X>1$, is shown  in blue, whereas the region excluded by cluster observations is the hatched one. We also  give the values of $\alpha_X$ and $m_A$ which yield the observed DM relic density assuming $T'/T$ ratios at freeze-out different from one (black dashed lines).} 
\label{ma-alpha-som}
\end{figure} 

\begin{figure}[t!]
\centering
\centering\includegraphics[width=0.65\textwidth]{3to2scan.pdf}
\caption{Values of the temperature ratio $T'/T$  at $T'>m_\eta$ (and after the connector has ceased to create HS particles) required in order to generate the measured DM abundance via the 3-to-2 \emph{dark freeze-out} (colored band) under the assumption of no kinetic equilibrium between the hidden and visible sectors.
The gray, red and blue lines correspond to $\sigma_{AA}/\ma=0.1$, 1 and 10 cm$^2/$g, respectively, so that the hatched light-blue region is excluded by the cluster bound, $\sigma_{AA}/\ma>1$~cm$^2/$g. The left-top white region is excluded by Lyman-$\alpha$ data.  We also show the values of $m_A$ and $\alpha_X$ which lead to \emph{reannihilation} and \emph{freeze-in} regimes rather than dark freeze-out. See text for details. 
}
\label{ma-alpha-som2}
\end{figure} 

\subsubsection{Invisible Decay of the SM scalar}

The HS increases the number of Higgs boson decay channels.
The new decay modes are into $\eta$ scalars and DM particles.
The latter contribute to the invisible decay of the Higgs boson, whereas the former  does it partially if subsequently the $\eta$ scalars, in addition to decay to (visible) SM particles, also decay into DM. The corresponding decay rates are
\begin{eqnarray}
\Gamma(h\to AA)&=&\frac{3g_X^2}{128\pi}\sqrt{\mh^2-4\ma^2}\frac{12 \ma^4 - 4 \ma^2 \mh^2 + \mh^4}{\ma^2\mh^2}\sin^2\beta\,,\\
%
\Gamma(h\to\eta\eta)&=&\frac{1}{128\pi}\sqrt{\mh^2-4\meta^2}\left[\frac{2\meta^2+\mh^2}{\ma\mh v}\right]^2\left[g_X v\cos\beta+2\ma\sin\beta\right]^2\sin^2\beta\,.
%
\end{eqnarray}
Moreover, all the decay widths of the Higgs boson into SM particles at tree-level decrease by a factor $\cos^2\beta$ compared to the SM ones.
%
For the $\eta$ scalar, the decay width into SM particles at tree-level is $\Gamma(\eta\to\text{SM SM})=\Gamma_\text{SM}(h\to\text{SM SM})|_{\mh\to\meta}\cdot\sin^2\beta$.  As for the $\eta$ decay width into DM particle, if kinematically allowed, it is given by
%
\begin{equation}
\Gamma(\eta\to AA)=\frac{3g_X^2}{128\pi}\sqrt{\meta^2-4\ma^2}\frac{12 \ma^4 - 4 \ma^2 \meta^2 + \meta^4}{\ma^2\meta^2}\cos^2\beta\,.
\end{equation}
%
%
In this work, we adopt the bound on the invisible Higgs branching ratio and on $\cos^2\beta$ obtained in the analysis of Ref.~\cite{Bechtle:2014ewa}, which accounts for all the
relevant experimental information on the Higgs boson properties, considering simultaneously a universal modification of the Higgs boson couplings to SM particles and the possibility of an invisible Higgs decay. By doing this, it is found that
\begin{equation}
\cos^2 \beta \left[ 1 - \text{Br}_\text{inv} \right] \gtrsim 0.81 \;\;\; 
\hspace{15pt}\text{with}\hspace{15pt}
\text{Br}_\text{inv} = \text{Br}(h\to A\,A)+\text{Br}(h\to\eta\,\eta)\,\text{Br}(\eta\to A\,A)^2\,
\end{equation}
for the case of no light mediator, where we are concerned with $m_A, m_ \eta \ll m_h/2$. This in turn gives a very strong bound on the mixing angle
\begin{equation}
\sin\beta \lesssim  10^{-4}\sqrt{{1\over \alpha_X }\cdot  {m_A \over \text{GeV}}}. \label{invi:Higgs}
\end{equation}
The situation of the light mediator case is different. First, due to its lightness, the mediator $\eta$ only decays to SM particles. Consequently, the decay of Higgs to $\eta$ is in practice \textit{visible} unless $\eta$ decays dominantly to neutrinos or the lifetime of $\eta$ is so long that it decays outside the detector. Moreover, for $m_A \ge m_h/2$, the other decay channel of Higgs into HS particles, $h\to A\,A$, is kinetically forbidden.  Therefore, if $\eta$ decays dominantly to charged fermions or photons  within the detector and $m_A \ge m_h/2$, there would be no sizable invisible decay of the Higgs boson, and thus no relevant bound on $\sin\beta$. Otherwise, a bound similar to Eq.~\eqref{invi:Higgs} holds.

\subsubsection{Boltzmann Equations for the 3-to-2 Annihilation and the Instantaneous Freeze-out Approximation}

In this appendix we assume that the dark and visible sectors have temperatures $T$ and $T'$ which are not necessarily equal. With this in mind, 
the evolution of the number densities $\n_i$ of the three DM particles $A_i$ are described by a system of three Boltzmann equations
{\small
\begin{eqnarray}
&&\frac{d\n_1}{dt}+3H\,\n_1=+\RR{1}{2}{3}{1}{1}\nonumber\\
&&-\RR{1}{2}{3}{2}{2}-\RR{1}{2}{3}{3}{3}\nonumber\\
&&-\RR{1}{1}{3}{1}{2}+\RR{2}{2}{3}{1}{2}\nonumber\\
&&+\RR{3}{3}{3}{1}{2}-\RR{1}{1}{2}{1}{3}\nonumber\\
&&+\RR{2}{2}{2}{1}{3}+\RR{2}{3}{3}{1}{3}\nonumber\\
&&-3\RR{1}{1}{1}{2}{3}-\RR{1}{2}{2}{2}{3}\nonumber\\
&&-\RR{1}{3}{3}{2}{3}\,,
\end{eqnarray}}
with two equivalent expressions for $\n_2$ and $\n_3$.
Here, $\neqq_i$ corresponds to the equilibrium densities and $\langle ijk\to lm\rangle\equiv\langle\sigma v^2\rangle_{ijk\to lm}$. 
 Due to the custodial symmetry the relation $\n\equiv \n_1=\n_2=\n_2$ holds and we find that 
$\NN{1}{2}{3}{1}{1}=\NN{1}{2}{3}{2}{2}=\NN{1}{2}{3}{3}{3}$, $\NN{1}{1}{1}{2}{3}=\NN{2}{2}{2}{1}{3}=\NN{3}{3}{3}{1}{2}$ and $\NN{1}{1}{3}{1}{2}=\NN{1}{1}{2}{1}{3}=\NN{2}{2}{3}{1}{2}=\NN{1}{2}{2}{2}{3}=\NN{1}{3}{3}{2}{3}=\NN{2}{3}{3}{1}{3}$. Thus the Boltzmann equations reduce to
\begin{equation}
\frac{d\n}{dt}+3H\,\n=\Big(-\NN{1}{2}{3}{1}{1}-\NN{1}{1}{1}{2}{3}-2\NN{1}{2}{2}{2}{3}\Big)\left(\n^3-\n^2\,\neqq\right)\,.
\end{equation}

As a result, total DM number density $N'=\n_1+\n_2+\n_3=3\,\n$ is given by
\begin{equation}
\frac{dN'}{dt}+3H\,N'=-\langle\sigma v^2\rangle_{3\to 2}\left(N'^3-N'^2\,{N'}^\text{eq}\right)\,,
\label{BE}
\end{equation}
where
\begin{equation}
\langle\sigma v^2\rangle_{3\to 2}\equiv\frac{\NN{1}{2}{3}{1}{1}+\NN{1}{1}{1}{2}{3}+2\,\NN{1}{2}{2}{2}{3}}{9}\,.
\label{sv32}
\end{equation}
%
 Following Ref.~\cite{Bernal:2015bla} to calculate the cross section in the non-relativistic limit, we find
\begin{equation}
\langle\sigma {v^2}\rangle_{3\to 2}=\frac{25\sqrt{5}\pi^2\,\alpha_X^3}{186624\ma^5}\,\frac{503295 \ma^8 + 592316 \ma^6 \meta^2 + 36188 \ma^4 \meta^4 - 156224 \ma^2 \meta^6 + 26209 \meta^8}{(\meta^2-4 \ma^2)^2 (\ma^2 + \meta^2)^2}\,.
\end{equation}


The Boltzmann Eq.~\eqref{BE} gives the DM number density as a function of time. Since we assume that the SM particles dominate the expansion of the Universe, we can trade the time variable $t$ for the temperature $T$ of the SM. By performing this change of variables we obtain
%
\begin{equation}
x\,H(x)\frac{dY(x)}{dx}=-s(x)^2\,Y(x)^2\,\langle\sigma v^2\rangle_{3\to 2} \, \big(Y(x)-Y^\text{eq}(x)\big)\,,
\label{BEY}
\end{equation} 
%
where $x\equiv \ma/T$ and $Y(x)\equiv N'/s(x)$. Notice that we define $Y(x)$ as a function of the SM quantities $x$ and $s(x)$, because it can be related to the today DM relic abundance by means of
%
\begin{equation}
\Omega_A = \frac{\ma\,N'}{\rho_c}=\frac{\ma\,s(\infty)\,Y(\infty)}{\rho_c}=\left(2.742 \cdot 10^8 \,\text{GeV}^{-1} \, h^{-2}\right) \, \ma \, Y(\infty)\,. 
\label{RelicDensity}
\end{equation}
%
 In this paper we use the following approximate solution of Eq.~\eqref{BEY}. 
After the freeze-out the DM density deviates from its equilibrium value. In fact,  as it becomes much greater, $ Y \gg Y^\text{eq}$, one can drop the $Y^{eq}$ term in Eq.~(\ref{BEY}), so that
%
\begin{equation}
x\,H(x)\frac{dY(x)}{dx}=-s(x)^2\,Y(x)^3\,\langle\sigma v^2\rangle_{3\to 2}\,.
\end{equation} 
%    
This equation admits the following analytical solution
%
\begin{equation}
\frac{1}{Y(\infty)^2} = \frac{1}{Y(\xf)^2} + 2\int^\infty_{\xf} \frac{s^2\,\langle \sigma v^2\rangle_{3 \to 2} }{x\, H} dx\,.
\end{equation}
%
Here $\xf$ corresponds to the freeze-out temperature,  to be determined below. In general, one expects $ Y(\infty) \ll Y(\xf)$ and therefore 
%
\begin{equation}
Y(\infty) = \left[ 2 \int^\infty_{\xf} \frac{s^2\,\langle \sigma v^2\rangle_{3 \to 2} }{x\, H} dx\right]^{-1/2}\,.
\end{equation}
%
%
%
Now, since the DM particles are non-relativistic at freeze-out, the cross section $\langle \sigma v^2 \rangle_{3\to 2}$ is independent of the temperature.  It is therefore possible to conclude that in order to account for the observed DM relic density, Eq.~\eqref{RelicDensity}, one needs
%
\begin{equation}
\langle \sigma v^2 \rangle_{3\to2} \approx \left( 8.65\,\text{GeV}^{-5}\right) \,\xf^4 \, g_{*\text{FO}}^{-1.5} \left(\frac{1\, \text{GeV}}{\ma} \right)^2\,,
\label{FOconditionbis}
\end{equation}  
%%
%
where $g_{*\text{FO}}$ corresponds to the number of relativistic degrees of freedom at the moment of the freeze-out.
 Note that it is the SM temperature at the freeze-out which enters in this formula and not the DM one. 

In order to estimate $\xf$, it is necessary to establish when the annihilation rate per particle  $(\neqq)^2 \langle \sigma v \rangle_{ 3\to 2}$ drops below the expansion rate of the Universe. Using Eq.~\eqref{FOconditionbis} it is found that this happens when freeze-out temperatures satisfy 
%
\begin{equation}
\xpf = 22.3 - \ln \left[\left(\frac{\xpf}{\xf}\right)^3\left(\frac{100 \,\text{MeV}}{\ma}\right)\left(\frac{g_{*\text{FO}}}{10}\right)\left(\frac{\xpf}{22.3}\right)^{-1.5}\right]\,.
\label{xpf}
\end{equation}
Injecting the value of $x'_\text{FO}$ one needs for a given value of the entropy ratio $\xi$ according to Eq.~\eqref{3to2:decouple}, this equation gives the value of $x_\text{FO}$.

\subsubsection{Conclusions}

within this model the solution of the small scale problems is incompatible with the ordinary freeze-out scenario.
Nevertheless two alternative production scenarios do work easily.
These scenarios are: $(a)$ dark freeze-out via 3-to-2 annihilation of a  HS colder than the SM, and $(b)$ freeze-in via the exchange of a light mediator.  

First let us summarize what happens along the various regimes for the case of no light mediator, i.e.~{\it considering a 3-to-2 annihilation}. 
In this case, the small-scale structure problems and the Higgs invisible decay constraints require sub-GeV DM with sizable self-interactions and a relatively small connector.
The outcome is

\begin{itemize}
\item \underline{Portal interaction freeze-out}: Since a sub-GeV DM particle can annihilate via the Higgs portal into a couple of SM particles  only at a very suppressed rate (due to the mixing angle and the Yukawa coupling), this scenario
is not viable. 

\item \underline{Dark freeze-out with $T=T'$}: A scenario with DM annihilations via 3-to-2 interactions, assuming that the DM temperature $T'$ and the SM temperature $T$ are equal, is not feasible because: $(i)$ one can not get simultaneously the observed relic density and significant self-interactions with perturbative $\alpha_X$ couplings (see Fig.~\ref{ma-alpha-som});
$(ii)$ at the moment of the DM freeze-out, the Higgs portal is too suppressed to maintain the kinetic equilibrium between the two sectors, giving rise to tension with the formation of cosmological structures.

\item \underline{Dark freeze-out with $T'<T$}: This scenario solves the previous two problems.
On the one hand, $T'<T$ implies a less populated HS and  thus smaller annihilation cross sections are needed to produce the observed relic density.
 Accordingly, perturbative values of $\alpha_X$ are compatible with both the DM abundance  constraint and the self-interaction hypothesis (e.g. Fig.~\ref{ma-alpha-som}).
On the other hand, if $T'<T$ at the moment of the freeze-out, structure formation constraints are naturally fulfilled, simply because DM is colder than the SM particles.
On top of that, this regime can also satisfy all other experimental constraints previously mentioned.
Fig.~\ref{fig:caseB} shows the way the relic density is obtained in this case as a function of $T$ and $T'$ for an example of successful set of parameters.
In particular, when the 3-to-2 annihilations become efficient, the HS heats up with respect to the SM sector. 
The parameter space allowed in this scenario is depicted in Fig.~\ref{ma-alpha-som2}, which corresponds to DM masses between a few keV and $\sim100$\,MeV.


\item \underline{Reannihilation}: This scenario requires that at the time when the HS interactions get Boltzmann suppressed (i.e. $T'\lesssim m_A$), the connector still creates HS particles. Due to the low DM mass range required by DM self-interactions, in the HVDM model reannihilation never takes place. This is because the (mixing angle and Yukawa suppressed) Higgs portal ceases to be active as soon as $T$ goes below $\sim 10$\,GeV. One could think about considering tiny values for $T'/T$ to overcome this difficulty but this would be incompatible with  the observed DM abundance.
It must be stressed however that for other kind of portals not suppressed at low temperatures (for instance a $Z'$ portal), the reannihilation could work  similarly to the way the dark freeze-out with $T'<T$ does.

\item \underline{Freeze-in}: This regime requires a HS that never thermalizes within itself. This implies a value of $\alpha_X$ which leads to self-interactions too feeble to  solve small-scale problems, unless one considers very light DM ($3$~keV $\lesssim m_A\lesssim10$~keV) at the verge of being too hot to be allowed.



\end{itemize}


The discussion of the regimes for the case with a light mediator differs in many aspects. In this case annihilations  proceed via 2-to-2 processes, and  the self-interaction hypothesis requires a mediator mass below $\sim 100$\,MeV with the DM particle several orders of magnitude heavier, which leads to the following conclusions:

\begin{itemize}
\item \underline{Portal interaction freeze-out}: This scenario does not work. 
On the one hand, for $\ma\lesssim 1$\,GeV the DM annihilates mainly into the HS and not into SM pairs as required in this scenario.
On the other hand, direct detection experiments exclude DM heavier that $\sim 1$\,GeV because of the strong enhancement of the DM-nucleon cross section (due to the lightness of the mediator).


\item \underline{Dark freeze-out with $T=T'$}: In this case DM annihilates through $AA\to\eta\eta$ or $A\eta$.
The thermalization condition $T=T'$ implies that the connector interaction should be sizable. However, direct detection bounds and cosmological observations require a much smaller connector,  basically excluding this regime.

\item \underline{Dark freeze-out with $T'<T$}: Unlike the case without light mediators,  most of the parameter space in this regime turns out to be excluded. Generally speaking this stems from two facts. First, this scenario predicts a relatively large annihilation cross section from the requirement that the HS thermalizes. Second it predicts  yields such that $Y_\eta\gg Y_A$. All this  leads to strong tensions with BBN, CMB and $X$-ray constraints. 
Details can be found in Appendix~\ref{sec:AppendixC}. 

\item \underline{Reannihilation}: This regime is analogous to the previous one, in the sense that it also requires a relatively large annihilation cross section and gives $Y_\eta\gg Y_A$.
As a consequence, as the previous regime it is excluded except in corners of the parameter space.


\item \underline{Freeze-in}: Finally, and unlike all the other light mediator regimes above, the freeze-in regime can easily work. This is due to the following  three facts. First, since this scenario is based on the assumption that the HS never reaches thermal equilibrium, it requires smaller values of $\alpha_X$ and $\sin\beta$, which allow to fulfill the direct detection constraints. Second, 
this regime decouples the $\alpha_X$-driven self-interaction  hypothesis from production of the DM, which is $\alpha_X$-independent.
Finally, unlike the dark freeze-out regimes, the freeze-in scenario naturally predicts $\Omega_\eta/\Omega_A\ll 1$, which permits to easily satisfy the $X$-ray and CMB constraints.
Fig.~\ref{fig:caseD} shows an example of successful freeze-in evolution of the DM relic density, together with the mass range needed in this case.

\end{itemize}



To sum up very shortly, the production of self-interacting DM in the early Universe can be
achieved by considering a DM sector which is not in thermal equilibrium with the SM bath.
We considered this possibility in the context of the particularly simple HVDM model. We are not aware of a simpler model that can simultaneously address all the issues discussed here. Moreover, many
of the conclusions we came to in this particular model would certainly remain valid for other
models where DM interacts with the SM via a portal.

\subsection{1704.05359 - WIMP miracle of the second kind (Heikinheimo, Tenkanen, Tuominen)}

\subsection{1707.01434 - Vector SIMP dark matter (Mambrini, Pierre et al.)}

\subsubsection{Vector SIMP dark matter}\label{sec:relic}


Having established the interactions of the framework, we now address the cross section for the dark matter relic abundance and self-scatterings.
We first determine the relic density of dark matter from $3\to2$ processes in Section~\ref{ssec:SIMP}, and discuss the role of additional forbidden annihilation channels in Section~\ref{ssec:forb}.




\subsubsection*{SIMP channels}\label{ssec:SIMP}

Here we compute the relic density assuming the $3\to2 $ annihilation processes are the dominant number-changing processes. In the presence of an isospin symmetry for the vector dark matter, all components of dark matter have the same mass, and can be treated as identical particles.
Assuming the dark matter remains in kinetic equilibrium with the SM until the time of freeze-out,
the Boltzmann equation for the vector dark matter is given by~\cite{Hochberg:2014dra}
\bea
\frac{d n_{\rm DM}}{dt}+ 3 H n_{\rm DM}&=& -\Big(\langle\sigma v^2\rangle_{3\rightarrow 2}-\langle\sigma v^2\rangle^h_{3\rightarrow 2}\Big) \Big(n^3_{\rm DM}- n^2_{\rm DM}n^{\rm eq}_{\rm DM}\Big) \nonumber \\
&&-\langle\sigma v^2\rangle^h_{3\rightarrow 2}\Big(n^3_{\rm DM}- n_{\rm DM}(n^{\rm eq}_{\rm DM})^2 \Big)\,.
\eea
Here, the thermally averaged $3\rightarrow 2$ annihilation cross-section (away from a resonance) is given by
\bea
\langle\sigma v^2\rangle_{3\rightarrow 2}&=&\frac{25\sqrt{5}g_X^6}{23887872\pi m_X^5}\frac{1}{(m_{h_1}^2-4m_X^2)^2(m_{h_1}^2+m_X^2)^2} \bigg(14681m_{h_1}^8-87520m_{h_1}^6m_X^2 \nonumber \\
&&+21004m_{h_1}^4m_X^4+327580m_{h_1}^2m_X^6 +290775m_X^8\bigg) +\langle\sigma v^2\rangle^h_{3\rightarrow 2}
\label{3to2}
\eea
with
\bea
\langle\sigma v^2\rangle^h_{3\rightarrow 2}=  \frac{\sqrt{5}g_X^6m^{16}_{h_1}}{80621568\pi m_X^{10}} \frac{(1-m^2_{h_1}/(16 m^2_X) )^{1/2} }{(m_{h_1}^2-4m_X^2)^{7/2}(m_{h_1}^2+2m_X^2)^2}\bigg(C_1+\frac{2C_2 m^4_{h_1}}{(m^2_{h_1}-7m^2_X)^2} \bigg)  
\eea
where $C_1$ and $C_2$ are dimensionless quantities given in Eqs.~(\ref{C1}) and (\ref{C2}), respectively.  We note that the first term in $\langle\sigma v^2\rangle_{3\rightarrow 2}$ stems from $XXX\rightarrow XX$ channels and $\langle\sigma v^2\rangle^h_{3\rightarrow 2}$ due to $XXX\rightarrow X h_1$ channels contributes only for $m_{h_1}<2m_X$, becoming dominant near the resonance at $m_{h_1}=2m_X$. On the other hand, $XXX\rightarrow h_1 h_1$ channels are $p$-wave suppressed so they are not included here.  
Additional terms that give an approximate resonance when $m_{h_1}= 3 m_X$ are present, but as they are $p$-wave suppressed they are always subdominant and hence can be neglected. Further details of the $3\rightarrow 2$ cross section and discussion of the Boltzmann equation can be found in Appendix~\ref{app:xsec}.




In the instantaneous freeze-out approximation, the relic abundance for $3\rightarrow 2$ annihilation is found to be
\bea
\Omega_{\rm DM}  \simeq \frac{m_X s_0/\rho_c}{s({m_X})^2 / H(m_X)} \frac{x_f^2}{\sqrt{\langle\sigma v^2\rangle_{3\rightarrow 2}}}\,,
\eea
where ${s_0/\rho_c \simeq 6\cdot 10^8 /\rm GeV}$ is the ratio of the entropy density today to the critical density, $s(m_X)$ is the entropy density at $T= m_X$, and $H(m_X)$ is the Hubble rate at $T= m_X$. Here $x_f=m_X/T_f$ indicates the freezeout temperature, which is typically $x_f \in [15,20]$ for $3\to 2 $ freezeout.
For $m_{h_1} \gtrsim 3 m_X$, the Higgs contributions to the cross-section effectively decouples, and we have
\bea
\Omega_{\rm DM} \simeq 0.33 \left( \frac{x_f}{20}\right)^2 \left( \frac{10.75}{g_*}\right)^{3/4} \left(\frac{m_X/\alpha_X }{100~ \rm MeV} \right)^{3/2}\,.
\eea


\begin{figure}[t!]
  \begin{center}
      \includegraphics[height=0.45\textwidth]{figures/relic1}\\
             \includegraphics[height=0.45\textwidth]{figures/relic2}
      \includegraphics[height=0.45\textwidth]{figures/relic3}
   \end{center}
  \caption{The parameter space of vector SIMP dark matter in the $m_X$ vs. $\alpha_X\equiv g^2_X/(4\pi)$ (top) or $m_{h_1}$ (bottom), when considering $3\to2$ annihilation channels only. The Planck $3\sigma$ measurement of the relic density is show in red in all panels. Contours of the self-scattering cross section of $\sigma_{\rm self}/m_X=0.1,1,10\,{\rm cm^2/g}$ are shown in the dotted, dashed and dot-dashed curves, respectively.  We have chosen $m_{h_1}=4m_X$ on top and $\alpha_X=1, 2$ on bottom. The shaded gray regions in the lower panels are where other $2\rightarrow 2$ channels dominate over $3\to2$ processes. }
  \label{relic}
\end{figure}

In Fig.~\ref{relic} we depict the parameter space in which the measured dark matter relic density is obtained within $3\sigma$ (red region) for $\alpha_X\equiv g^2_X/(4\pi)$ ($m_{h_1}$) and $m_X$ in the upper (lower) panel. For illustration, the top panel shows the results for dark Higgs mass of $m_{h_1}=4m_X$ where no resonance enhancement is present, while in the bottom panel we fix $\alpha_X=1, 2$ and vary $m_X$ and $m_{h_1}$.

In addition to $3\to2$ annihilations, the vector SIMP dark matter undergoes self-scattering processes, which are constrained by the bullet cluster~\cite{Clowe:2003tk,Markevitch:2003at,Randall:2007ph} and by elliptical halo shapes~\cite{Rocha:2012jg,Peter:2012jh}. Away from a resonance, the self interacting cross-section is
\bea
\sigma_{\rm self}
&=&\frac{g^4_X}{1152\pi m_{h_1}^4m_X^2(m_{h_1}^2-4m_X^2)^2}
\Big(520m_{h_1}^8-4208m_{h_1}^6m_X^2+8801m_{h_1}^4m_X^4 \nonumber \\
&&-1200m_{h_1}^2m_X^6+320m_X^8\Big)\,.
\eea
A simple approximation can be derived in the limit $m_{h_1} \gg m_X$ : \begin{equation}
\dfrac{\sigma_\text{self}}{m_X}\simeq \frac{65 \pi  \alpha _X^2}{9 m_X^3} \simeq 5 \alpha_X^2 \Big( \dfrac{m_X}{100\text{ MeV}} \Big)^{-3}  \text{ cm}^2 / \text{g} \qquad \qquad [m_{h_1} \gg m_X]
\end{equation}
%
Contours of the self-scattering cross section obeying $\sigma_{\rm self}/m_X=0.1,1,10\,{\rm cm^2/g}$ are shown in Fig.~\ref{relic} in dotted, dashed and dot-dashed lines, respectively.


We learn that away from a resonance region, vector SIMP $3\to2$ dark matter consistent with self-scattering constraints points to dark matter masses of $m_X\gtrsim {\cal O}(100~{\rm MeV})$ and strong couplings of $\alpha_X\gtrsim 1$. Indeed, strong coupling is a frequent common feature in SIMP dark matter models~\cite{Hochberg:2014dra,Lee:2015gsa,Choi:2015bya,Hochberg:2015vrg,Choi:2016tkj,Hambye:2009fg,Hambye:2008bq,Bernal:2015ova,Cline:2017tka}, though exceptions can arise ({\it e.g.} on resonance~\cite{Choi:2016hid,Choi:2017mkk}).  
Close to the resonance region, the relic density is sensitive to the dark Higgs mass, and the viable parameter space is broadened further to include larger DM masses at fixed dark gauge coupling, or smaller dark gauge couplings for fixed DM masses.

We comment that the strong gauge coupling leads to a question on the potential breakdown of perturbativity in relic density calculation. In our case, however, the $SU(2)_X$ gauge symmetry is completely broken by the VEV of the dark Higgs, and there are no light particles below the confinement or symmetry breaking scale ({\it i.e.}\/, vector SIMP mass). Therefore, given that there is no phase transition separating the Higgs phase and confining phase, namely, the complementarity between the Higgs and confining phases~ \cite{Fradkin:1978dv,Banks:1979fi,tHooft:1979yoe,Susskind:1979up,Raby:1979my,Georgi:2016qbt}, the Higgsed theory can be pushed into regions where perturbativity is questionable. Closer inspection of the issue of complementarity may be worthwhile, though is beyond the scope of this paper. 

As the dark Higgs mass approaches the DM mass, when $m_X< m_{h_1}\lesssim 1.5 m_X$, forbidden $2\to2$ annihilation channels contribute significantly to the relic density and must be included as well; we study this in the next subsection. (The regions in which $2\to2$ processes dominate the relic density are shown in shaded gray in Fig.~\ref{relic}.) As we will see, the self-scattering rate is reduced in this case, allowing smaller dark matter masses consistent with observational constraints.


\subsubsection*{Forbidden channels}\label{ssec:forb}


When the dark Higgs is slightly heavier than the dark matter, forbidden $2 \rightarrow 2$ channels such as $X_iX_i\rightarrow h_1 h_1$ and $X_iX_j\rightarrow X_k h_1$---although kinematically inaccessible at zero temperature---can be important in determining the relic density at the time of freeze-out~\cite{Griest:1990kh,DAgnolo:2015ujb}.  For $m_X\lesssim m_{h_1}\lesssim2(1.5)m_X$, new $3\rightarrow 2$ channels such as $XXX\rightarrow X h_1 (h_1 h_1)$ open up as well so they have been already included in Fig.~\ref{relic}.  Here we discuss the effects of the forbidden channels on the relic abundance and identify the parameter space of vector SIMP dark matter that is consistent with the observed relic density when including these effects.
(This will be particularly relevant when kinetic equilibrium between the SIMP and SM sectors is obtained via the Higgs portal, as will become evident in Section~\ref{ssec:higgsportal}.)


Assuming that the forbidden channels are dominant,  the approximate Boltzmann equation is given by
\bea
\frac{dn_{\rm DM}}{dt}+3Hn_{\rm DM}&\approx &-\frac{2}{3}\langle\sigma v\rangle_{ii\rightarrow h_1 h_1} n^2_{\rm DM}+6\langle\sigma v\rangle_{h_1 h_1\rightarrow ii} (n^{\rm eq}_{h_1})^2  \nonumber \\
&&- \frac{1}{3}\langle\sigma v\rangle_{ij\rightarrow k h_1} n^2_{\rm DM} +\langle\sigma v\rangle_{k h_1\rightarrow ij}n^{\rm eq}_{h_1} n_{\rm DM}\,,
\eea
where we have assumed that $h_1$ maintains chemical and thermal equilibrium with the SM bath throughout freezeout. See the full Boltzmann equations in Eq.~(\ref{fullBoltz}).  
Detailed balance conditions at high temperature determine the annihilation cross sections for the forbidden channels in terms of the unforbidden channels,
\bea
\langle\sigma v\rangle_{ii\rightarrow h_1 h_1} &=& \frac{9(n^{\rm eq}_{h_1})^2}{(n^{\rm eq}_{\rm DM})^2} \,\langle\sigma v\rangle_{h_1 h_1\rightarrow ii}
= (1+\Delta_{h_1})^3 e^{-2\Delta_{h_1}x}  \,\langle\sigma v\rangle_{h_1 h_1\rightarrow ii}\,, \label{dbal1} \\
\langle\sigma v\rangle_{ij\rightarrow k h_1} &=& \frac{ 3n^{\rm eq}_{h_1}}{n_{\rm DM}^{\rm eq}}\, \langle\sigma v\rangle_{k h_1\rightarrow ij} = (1+\Delta_{h_1})^{3/2} e^{-\Delta_{h_1}x} \,  \langle\sigma v\rangle_{k h_1\rightarrow ij}\,,  \label{dbal2}
\eea
with $\Delta_{h_1}\equiv (m_{h_1}-m_\chi)/m_\chi$.   The cross section formulas for the allowed $2\rightarrow 2$ channels in the RHS above are given in Appendix~\ref{app:xsec}.

Denoting the allowed $2\to2$ cross sections in the RHS above by $ \langle\sigma v\rangle_{k h_1\rightarrow ij} =a$ and $ \langle\sigma v\rangle_{h_1 h_1\rightarrow ii}=b$, the DM abundance is found to be~\cite{DAgnolo:2015ujb}
\be
Y_{\rm DM}(\infty)\approx \frac{x_f}{\lambda}\, e^{\Delta_{h_1}x_f} \, f(\Delta_{h_1},x_f)
\ee
with 
\bea
f(\Delta_{h_1},x_f)&=& \bigg[ \frac{1}{3} a (1+\Delta_{h_1})^{3/2}\Big(1-(\Delta_{h_1} x_f) \, e^{\Delta_{h_1}x_f} \int^\infty_{\Delta_{h_1} x_f} dt\, t^{-1} e^{-t} \Big) \nonumber \\
&+& \frac{2}{3} b(1+\Delta_{h_1})^3 e^{-\Delta_{h_1}x_f}\Big(1-2(\Delta_{h_1}x_f)\,e^{2\Delta_{h_1} x_F} \int^\infty_{2\Delta_{h_1} x_f} dt\, t^{-1} e^{-t} \Big)  \bigg]^{-1}\,,
\eea
resulting in the relic density
\be
\Omega_{\rm DM}h^2 = 5.20\times 10^{-10}\,{\rm GeV}^{-2} \Big(\frac{g_*}{10.75} \Big)^{-1/2} \Big(\frac{x_f}{20} \Big)\, e^{\Delta_{h_1} x_f} f(\Delta_{h_1},x_f)\,.
\ee
In general, however, one must account simultaneously for both the $3\rightarrow 2$ processes and the $2\rightarrow 2$ forbidden channels in determining the dark matter relic abundance.

\begin{figure}
  \begin{center}
  \includegraphics[height=0.45\textwidth]{figures/fdm}
      \includegraphics[height=0.45\textwidth]{figures/fdmsimp}
   \end{center}
  \caption{Dark matter relic density as a function of $\Delta_{h_1}=(m_{h_1}-m_X)/m_X$, for forbidden channels only ({\bf left}) and both forbidden and SIMP channels ({\bf right}). The measured relic density is shown by the purple curve. We show the results for various illustrative values of coupling and mass: $\alpha_X=0.01,0.1,1$ and $m_X=0.1\,{\rm MeV}, 1\,{\rm GeV}$.}
  \label{fdm2}
\end{figure}

In Fig.~\ref{fdm2}, we show the dark matter relic density as a function of $\Delta_{h_1}=(m_{h_1}-m_X)/m_X$, first when including only forbidden channels ({\bf left panel}) and then when taking both forbidden and SIMP channels into account ({\bf right panel}). We have varied $\alpha_X$ and $m_X$ between $0.01-1$ and $10\;{\rm MeV}-1\,{\rm GeV}$, respectively.
We learn that forbidden channels play an important role for $\Delta_{h_1}\lesssim 0.5$, where the observed relic density can be achieved over a broad range of couplings $\alpha_X$ and masses $m_X$. As the mass difference increases, $3\to2$ SIMP annihilations begin dominating the relic abundance as a saturated value for mass differences $\Delta_{h_1}\gtrsim 0.5$. We note that the importance of the forbidden semi-annihilation channels for $\Delta_{h_1}\lesssim 0.5$, in contrast to the naive expectation from the Boltzmann suppression factors of $\Delta_{h_1}\lesssim 1$, is due to a large numerical factor in the SIMP $3\to2$ annihilation cross section.


\subsubsection{Kinetic equilibrium}\label{sec:portal}


In order of the SIMP mechanism to be viable, we require that the SIMP sector efficiently dumps entropy into the SM bath. In the proposed framework, this can be achieved either by a Higgs or $Z'$ portal between the vector SIMPs and SM particles. After a general discussion of the relevant Boltzmann equation in terms of the dark sector temperature and the requirement of equilibration in Section~\ref{ssec:boltz}, we study the Higgs portal in Section~\ref{ssec:higgsportal} and the $Z'$ portal in Section~\ref{ssec:Zprimeportal}.


\subsubsection*{Equilibration conditions}\label{ssec:boltz}

Following Ref.~\cite{Kuflik:2015isi}, we find the decoupling temperature by comparing the rate of change in kinetic energy injected by the $3\to 2$ annihilations compared to the kinetic energy lost due to elastic scattering.  When the $3\to 2$ occurs, the mass of one dark particle is converted to the kinetic energy of the 2 outgoing particles. These  particles quickly scatter off the dark matter particles, and distribute the energy to the dark bath. Thus, the $3\to 2$  annihilations maintain chemical equilibrium in the DM gas, while releasing kinetic energy per particle
\beq
\dot{K}_{3\to 2} = m_{\rm DM}\, \frac{ \dot{n}_{\rm DM}}{n_{\rm DM}}\simeq  -m_{\rm DM}^2 H T^{-1}.\label{hubbleloss}
\eeq

Elastic scattering processes transfer this excess kinetic energy to the SM gas at a rate
\beq
\dot{K}_{\rm el} = \frac{1}{2 E_{p}} \sum_i \frac{g_i d^3 k_i}{(2\pi)^3 2 E_i} \frac{ d^3 k^\prime_i}{(2\pi)^3 2 k^\prime_i}  \frac{ d^3 p^\prime}{(2\pi)^3 2 p^\prime} \delta^4(p+k_i - p^\prime - k^\prime_i) \overline{|\mathcal{M}|^2} \left(E_{p} -E_{p^\prime} \right).
\eeq
Here, the sum is taken over the species $i$ in the relativistic plasma with initial(final) momentum $k(k^\prime)$, $p(p^\prime)$ is the dark matter initial(final) momentum. In the limit of $|{\vec k}|\ll m_{\rm DM}$, the change in kinetic energy can be written in terms of the momentum relaxation rate, $\gamma(T)$
\beq
\dot{K}_{\rm el} \simeq T \gamma(T)=\sum_i \frac{g_i}{6m_{\rm DM}} \int^\infty_0 \frac{d^3 {\vec k}}{(2\pi)^3} \, f_i (1\pm f_i) \frac{|{\vec k}|}{\sqrt{{\vec k}^2+m^2_i}}\,\int^0_{-4k^2} dt(-t) \frac{d\sigma_{Xi\rightarrow Xi}}{dt}, \label{elasticloss}
\eeq
where $t$ is the squared momentum transfer between DM and the relativistic species. The differential elastic scattering cross section is given by
\bea
 \frac{d\sigma_{Xi\rightarrow Xi}}{dt} =\frac{1}{64\pi m^2_{\rm DM}k^2}\, \overline{|{\cal M}_{Xi\rightarrow Xi}|^2}.
\eea

The decoupling occurs when the DM-to-SM energy transfer can no longer keep up with the kinetic energy production; equating Eq.~(\ref{hubbleloss}) with Eq.~(\ref{elasticloss}), we have
\beq
\gamma(T_{\rm KD}) \simeq H(T_{\rm KD}) \frac{m_{\rm DM}^2}{T_{\rm KD}^2} \label{eq:eqcond},
\eeq
where $H=0.33 g^{1/2}_* T^2/M_{\rm Pl}$ with $g_*=10.75$ the effective relativistic number of species for $1\,{\rm MeV}\lesssim T\lesssim 100\,{\rm MeV}$ and $M_{\rm Pl}=2\times 10^{18}$~GeV the Planck scale. In what follows we use Eq.~\eqref{eq:eqcond}, evaluated at $T_{\rm KD} = m_{\rm DM}/20$, to place a lower bound on the interactions between the vector SIMPs and the SM particles, needed to achieve the correct DM abundance. The ELDER DM curve~\cite{Kuflik:2015isi,Kuflik:2017iqs}, corresponds to $T_{\rm KD} \simeq m_{\rm DM}/15$, where the relic abundance is determined by the elastic scattering rate.

The dark matter can also thermalize with the SM, if the dark matter maintains equilibrium with the dark Higgs, while the dark Higgs maintains equilibrium with the SM bath via decay and inverse decays into SM fermions. The dark Higgs should be heavier than the dark $X$-bosons, or else the dark matter will efficiently annihilate into dark Higgs, effectively becoming a WIMP-like scenario. However, if the dark Higgs is much heavier than the dark matter, then the dark Higgs abundance will have been sufficiently depleted and it will not be able to maintain equilibrium between the two sectors.
This pushes the spectrum to a forbidden regime, $m_X< m_{h_1} \lesssim 1.5 m_X$, where the dark matter can annihilate into dark Higgses, but with a large Boltzmann suppression. At the time right before freezeout, both the semi-annihilation $XX \to X h_1 $ and self-annihilation $XXX \to XX$ processes will be active for large gauge coupling. The dark sector will be in thermal equilibrium with vanishing chemical potential. Thus in order for freezeout to occur one just needs to check that the dark Higgs can deplete the density in the dark sector fast enough up until freezeout,
\beq
n^{\rm eq}_{h_1}(T_{\rm FO}) \Gamma_{h_1 \to \rm SM} >  H(T_{\rm FO}) \left[n_{X }^{\rm eq}(T_{\rm FO})+ n_{h_1}^{\rm eq}(T_{\rm FO}) \right]\,. \label{eq:eqcond2}
\eeq
We use the above condition on the dark Higgs decay rate in the case that vector SIMPs are in kinetic equilibrium through the scattering with the dark Higgs.



\subsubsection*{Higgs portal}\label{ssec:higgsportal}


The coupling $\lambda_{\Phi H}$ present in Eq.~\eqref{eq:Vhiggs} leads to mixing between the SM and dark Higgs, which enables a Higgs portal between the dark and visible sectors.

In the presence of Higgs-portal induced mixing between the SM and dark Higgs, the SM Higgs can decay invisibly into a pair of dark matter particles, with decay rate given by Eq.~\eqref{eq:h2decay}:
\bea
\Gamma(h_2\rightarrow X X)= \frac{3\sin^2\theta m^3_{h_2}}{32 \pi v^2_X}\,\bigg(1-\frac{4m^2_X}{m^2_{h_2}}+\frac{12 m^4_X}{m^4_{h_2}} \bigg) \sqrt{1-\frac{4m^2_X}{m^2_{h_2}}}.
\eea
The combined VBF, $ZH$ and gluon fusion production of Higgs bosons at CMS leads to ${\rm BR}(h_2\rightarrow XX)<0.24$ at $95\%$ CL~\cite{Khachatryan:2016whc}, while the ATLAS bounds from the VBF~\cite{Aad:2015txa} and $ZH$~\cite{Aad:2014iia} modes give ${\rm BR}(h_2\rightarrow XX)<0.29$ and ${\rm BR}(h_2\rightarrow XX)<0.75$, respectively. These decays provide a strong constraint on the mixing: $\sin\theta \lesssim 10^{-5}$ for $\alpha_X\sim \mathcal{O}(1)$.


The mixing also induces direct couplings of the darks Higgs to the SM electron and muons, which in turn induces tree-level scattering of the SM of the leptons. However, the smallness of the electron Yukawa coupling and the Boltzmann-suppression of the muons at the time of freezeout combined with constraints on the Higgs invisible decay result in the elastic scattering being inefficient for thermalization.



\begin{figure}
  \begin{center}
      \includegraphics[height=0.46\textwidth]{figures/dHiggs4}
       \includegraphics[height=0.44\textwidth]{figures/mx-theta}
   \end{center}
  \caption{Vector SIMPs through the Higgs portal, with DM-dark Higgs scattering and dark Higgs-SM decays. {\bf Left:} Parameter space of $m_{h_1}$ vs. $\sin\theta$ for DM-dark Higgs scattering. The shaded purple regions indicate where kinetic equilibrium between the DM and dark Higgs fails.  {\bf Right:} Parameter space of $m_X$ vs. $\sin\theta$. The purple lines are the lower bounds on $\sin\theta$ from kinetic equilibrium for fixed ratios $m_{h_1}/m_X$.  {\bf In both panels:} the dashed black curves are the upper bounds on $\sin\theta$ from Higgs invisible decays.
  }
  \label{darkH}
\end{figure}

Alternatively, if the dark Higgs is fairly light, scattering between the vector dark matter and the dark Higgs can equilibrate the dark sector, with decays and inverse decays of the dark Higgs into SM particles completing the equilibration requirement between the SIMP and SM sectors.
The momentum relaxation rate from the elastic scattering of dark matter off of dark Higgs, $X_i h_1\rightarrow X_i h_1$, is given by
\bea\label{eq:eqHDM}
\gamma(T)_{h_1}= \frac{g_{h_1} g^4_X m^2_{h_1}}{12\pi^3 m_X (m_X+m_{h_1})^2}
\bigg(\frac{m^2_{h_1}-6m^2_X}{m^2_{h_1}- 4m^2_X} \bigg)^2 T^2\,e^{-m_{h_1}/T}
\eea
where $g_{h_1}=1$.  We note that the above result is valid for $m_{h_1}(m_{h_1}-2m_X)\gtrsim p^2_{\rm DM}\sim m^2_{\rm DM} v^2_{\rm DM}$.
Plugging this into the kinetic equilibrium condition Eq.~\eqref{eq:eqcond}, we find that equilibrium between the dark Higgs and the DM is effective in most of parameter space satisfying the dark matter relic abundance.

Simultaneously, kinetic equilibrium between the dark Higgs and the SM is maintained by decays and the inverse decays of the Higgs into a pair of SM fermions,
\bea\label{eq:eqHSM}
\Gamma(h_1\to f \bar f)=\frac{m^2_f m_{h_1} \sin^2\theta}{8\pi v^2} \left(1-\frac{4m^2_f}{m^2_{h_1}}\right)^{3/2}\,.
\eea
In Fig.~\ref{darkH}, we illustrate this second requirement of equilibration between the dark Higgs and the SM, as a function of $\sin\theta$ and $m_{h_1}$ ({\bf left}) or $m_X$ ({\bf right}) for fixed $m_X$ and $\alpha_X$ ({\bf left}) or fixed ratio $m_{h_1}/m_X$ ({\bf right}). The upper bound on the mixing angle from invisible Higgs decays is indicated by the dashed black curves in both panels. Here the active thermalization process comes primarily from decays into muons when kinematically accessible, and from electrons for smaller masses.

We learn that the Higgs portal is a viable mediator between vector SIMPs and the SM when the dark Higgs is close in mass to the DM. In this regime, $2\rightarrow 2$ forbidden (semi)-annihilations channels of DM and the dark Higgs, $X_i X_j\rightarrow X_k h_1 (h_1 h_1)$, can be active and are then important contributors in determining the dark matter relic density, as discussed in Section~\ref{ssec:forb}. In this case, the semi-annihilations are also active thermalization processes within the dark sector.

We note that current limits on Higgs mixing from rare kaon- and $B$-meson decays are weaker than the bound we impose from from the Higgs invisible decay. However future beam dump or fixed target experiments, such as SHiP at CERN SPS, have the potential to probe the Higgs mixing angle further down~\cite{Alekhin:2015byh}. The allowed parameter space for the Higgs portal to vector SIMPs could then be further probed as the invisible Higgs decay constraint improves.

Before ending this subsection, we remark that a Higgs portal coupling could allow in principle for the elastic scattering of relic vector SIMP dark matter with electrons in direct-detection experiments~\cite{Essig:2011nj,Graham:2012su,Lee:2015qva,Essig:2015cda,Hochberg:2015pha,Hochberg:2015fth,Hochberg:2016ntt,Essig:2016crl,
Derenzo:2016fse,Tiffenberg:2017aac,Essig:2017kqs}.  For $m_e, m_X,m_{Z'}\gg p_{\rm DM}\simeq m_X v_{\rm DM}$, the DM-electron direct detection scattering cross section via the Higgs portal is given by
\bea
\sigma_{\rm DD}&=&\frac{\alpha_X\sin^2\theta\cos^2\theta m^4_e m^2_X}{v^2 (m_e+m_X)^2}\left(\frac{1}{m^2_{h_1}}-\frac{1}{m^2_{h_2}}\right)^2\nonumber  \\
&\approx & 4\times 10^{-50}\,{\rm cm}^2 \left(\frac{\alpha_X}{2}\right)\left(\frac{\sin\theta}{10^{-4}}\right)^2\left(\frac{1.2}{m_{h_1}/m_X}\right)^4 \left(\frac{100\,{\rm MeV}}{m_X}\right)^4\,.
\eea
The small electron Yukawa coupling suppresses the cross section substantially, yielding a currently unconstrained spin-independent direct detection cross section.

\subsection{1801.03089 - Prospects for indirect detection of frozen-in dark matter (Heikinheimo, Tenkanen, Tuominen)}

\subsection{1805.01473 (CSI) - Super-cool Dark Matter (Hambye, Strumia, Teresi)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Super-cooling}
In dimension-less models, due to the absence of quadratic terms and vacuum stability (i.e.\ positive scalar quartics),
thermal effects 
%We instead assume that
%at large temperature, thermal effects 
select, as the Universe cools down, the false vacuum where all scalars
(in particular the dilaton $s$ and the Higgs $h$) have vanishing vacuum expectation values. Around this vacuum,
all particles are massless, including DM.
The energy density of the Universe receives two contributions:
from radiation, $\rho_{\rm rad}(T)= \sfrac{g_* \pi^2 T^4}{30}$,
and from the vacuum energy of the false vacuum $V_\Lambda >0$.
We assume that the true vacuum has a nearly zero vacuum energy, as
demanded by the observed small cosmological constant.


While the Universe cools,
the vacuum energy starts dominating over radiation at some temperature $T = T_{\rm infl}$
starting a phase of thermal inflation with Hubble constant $H$, such that
$V_\Lambda$ determines $ T_{\rm infl}$ and $H$ as
\begin{equation}\label{eq:TinflH}
  \frac{g_* \pi^2 T^4_{\rm infl}}{30} =  V_\Lambda = \frac{3H^2M_{\rm Pl}^2}{8\pi}
\end{equation}
where $g_*$ is the number of relativistic degrees of freedom just before inflation starts.
We denote as $a_{\rm infl}$ the scale factor of the Universe at this stage
and write ${\cal O}(1)$ factors in Boltzmann approximation (correct within $\pm10\%$)
given that DM might be bosonic or fermionic.


During this phase DM is massless and thereby remains coupled, rather than
undergoing thermal freeze-out at $T \sim T_{\rm dec}$ as e.g.\ in~\cite{1507.08660}.
All particles, including DM, undergo super-cooling:
the scale factor of the Universe grows as $a = a_{\rm infl} e^{Ht}$, and the temperature
drops as $T = T_{\rm infl} a_{\rm infl}/a$.






Super-cooling ends at some temperature $T_{\rm end}$ with a phase transition towards 
the true vacuum at $\med{s},\med{h}\neq 0$ ---
at the end of this section we will discuss how this happens in the models of interest.
During thermal inflation, the scale factor of the Universe inflates  by a factor
$e^N = \sfrac{T_{\rm infl}}{T_{\rm end}} $.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Reheating}
After the first-order phase transition to the true vacuum, the  various particles, including DM, become massive, and
the energy density $V_\Lambda$ stored in the scalars
is transferred to particles, reheating the Universe.
If the energy transfer  rate  $\Gamma$ is much faster than the Hubble rate $H$,
the reheating temperature is $g_{\rm RH}^{1/4}
T_{\rm RH}= g^{1/4}_* T_{\rm infl}$,
where $g_{\rm RH}$ is the number of reheated degrees of freedom.
Otherwise the scalars, before decaying, undergo a period of oscillations and the reheating temperature is lower.
%We approximate this process assuming that the inflaton $s$ has a decay rate $\Gamma$.
During this period, the scalars dilute as matter.
%such that in this fase $\rho_{\rm DM}/\rho_{\rm sca}$ stays constant.
When scalars finally decay, their remaining energy density $\rho_{\rm sca}$
becomes radiation with reheating temperature 
\beq T_{\rm RH}\approx T_{\rm infl} \min(1,\Gamma/H)^{1/2}.\eeq
The final DM abundance $Y_{\rm DM}= n_{\rm DM}/s$
(where $s = 2\pi^2 g_* T^3/45$ is the entropy density)
receives two contributions: 
%from super-cooling and possibly from thermal recoupling
\beq Y_{\rm DM} \approx  Y_{\rm DM}|_{\rm super-cool} +Y_{\rm DM}|_{\rm sub-thermal}.\label{twopopulations}\eeq
The super-cool contribution to the DM abundance is what remains
of the original  population of formerly massless DM in thermal equilibrium,
suppressed by the the dilution due to thermal inflation
\beq \label{eq:Ysc}
Y_{\rm DM}|_{\rm super-cool} =  Y^{\rm eq}_{\rm DM}   \frac{T_{\rm RH}}{T_{\rm infl}}
 \left(\frac{T_{\rm end}}{T_{\rm infl}}\right)^3,\qquad
 Y^{\rm eq}_{\rm DM}  =\frac{45g_{\rm DM}}{2\pi^4 g_*}  
 %\color{red}=\frac{\zeta(3) 45 g_{\rm DM}}{2\pi^4 g_*(T_{\rm infl})}  
 . \eeq
The factor  $T_{\rm RH}/T_{\rm infl}$ arises taking into account that
the energy stored in the oscillating inflaton dilutes as matter (rather than as radiation)
between the end of inflation and reheating, when it is finally converted to radiation. 


%\DT{We get: \\
%at the beginning of the oscillations $\rho_{DM} = M_X \frac{\zeta(3) g_{DM} T_{\rm end}^3}{\pi^2}$ because now the mass is $M_X$ and $\rho_s = V_{\Lambda} = \frac{g_*(T_{\rm infl}) \pi^2 T_{\rm infl}^4}{30}$ by definition of $T_{\rm infl}$ ;\\
%at the end: $\rho_{DM} = M_X Y_{DM}|_{\rm super-cool} \frac{2 \pi^2 g_*(T_{RH}) T_{RH}^3}{45}$ by definition of $Y_{DM}|_{\rm super-cool}$ and $\rho_s = \frac{g_*(T_{RH}) \pi^2 T_{RH}^4}{30}$ because of reheating. Imposing that $\rho_{DM}/\rho_{s}$ stays constant during the oscillations (as written above), we get
%\begin{equation}
%Y_{\rm DM}|_{\rm super-cool} =  Y^{\rm eq}_{\rm DM} \, \frac{T_{RH}}{T_{\rm infl}}
% \left(\frac{T_{\rm end}}{T_{\rm infl}}\right)^3,\qquad
% Y^{\rm eq}_{\rm DM}  =\frac{\zeta(3) 45 g_{\rm DM}}{2\pi^4 g_*(T_{\rm infl})}  
%\end{equation}
%}


  
The second contribution is the population of DM particles which can be produced from the thermal bath, through scattering effects, after reheating.\footnote{Production
during pre-heating was discussed in~\cite{1104.4791}.
Production during bubble collisions was discussed in~\cite{1211.5615}.}
% due to thermal scatterings.
If in this way DM has the time to thermalize again, i.e.\ if 
$T_{\rm RH} \gtrsim T_{\rm dec}$, the supercooled population is erased and this second population  reaches thermal equilibrium. 
In this case DM undergoes a usual freeze-out, leading to a relic density independent of whether there was previously a supercooling period.
%If instead DM decouples, erasing the super-cool contribution.
If instead $T_{\rm RH} \lesssim T_{\rm dec}$ the super-cool population remains basically unchanged, and the second population 
is produced with a sub-thermal abundance.
%and an extra thermal contribution is added.
This population is determined by the usual Boltzmann equation for
%be computed by considering the cosmological evolution of the DM abundance 
$Y_{\rm DM} = n_{\rm DM}/s$
in a radiation-dominated Universe, the same equation as the one that controls DM freeze-out.
In non-relativistic approximation
\beq  \frac{dY_{\rm DM}}{dz} = \frac{\lambda}{z^2} (Y^2 _{\rm DM}- Y_{\rm DM}^{\rm 2eq}),\qquad\hbox{where}\qquad
z = \frac{M_{\rm DM}}{T}.
\label{eq:Boltzf}\eeq
where
$ \lambda =
{M_{\rm Pl} M_{\rm DM} \langle\sigma_{\rm ann} v_{\rm rel}\rangle}\sqrt{\sfrac{\pi g_{\rm SM}}{45}}$
if DM annihilations have a cross section $\sigma_{\rm ann}$ dominated by $s$-wave scattering.
For $\lambda \gg 1$ freeze-out occurs at $T_{\rm dec} \approx M_{\rm DM}/ \ln\lambda$; otherwise DM never thermalizes again after reheating and the term proportional to $Y_{\rm DM}^{\rm 2eq}$ can be neglected.
Integrating eq.\eq{Boltzf} the regenerated DM population (starting from $T = T_{\rm RH}$) is
\beq \label{eq:YDMthermal}
Y_{\rm DM}|_{\rm sub-thermal} = \lambda \int_{z_{\rm RH}}^\infty \frac{dz}{z^2} Y_{\rm eq}^2 = \lambda  \, \frac{2025g_{\rm DM}^2}{128\pi^7 g_{\rm SM}^2}
e^{-2z_{\rm RH}} (1+2 z_{\rm RH}).\eeq

Summarising, the super-cool contribution dominates provided that $T_{\rm RH}\ll T_{\rm dec}$.
If DM interaction are small enough that it does not undergo kinetic recoupling, 
DM remains colder than in the freeze-out scenario: this has little observational implications~\cite{Gunn:1978gr};
the fact that super-cool DM forms smaller structures could give enhanced tidal fluctuations possibly observable
along the lines of~\cite{1710.06443}.
The super-cool population of eq.\eq{Ysc} does not depend on DM properties
(provided that initially, before supercooling, it was in thermal equilibrium), but only on the
amount of super-cooling.
As we will see below, eq.\eq{Ysc} matches the desired DM abundance provided that $T_{\rm end}$
is a few orders of magnitude below $T_{\rm RH}$. If instead  $T_{\rm RH} \lesssim T_{\rm dec}$, an additional non-thermal DM population is generated after reheating which can also lead to the desired relic density.
%
%The DM abundance remains sub-thermal if $T_{\rm RH} \circa{<}M/\ln\lambda$. 
%In such a case the final DM abundance is
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The dark matter abundance}

\begin{figure}[t]
\includegraphics[width=0.47\textwidth,height=0.45\textwidth]{m_g_phenoall.pdf}\qquad
\includegraphics[width=0.47\textwidth,height=0.47\textwidth]{evo.pdf}
\caption{\em  {\bf Left:}
The observed DM abundance is reproduced along the solid curves, computed for different values
of the uncertain QCD factor $\langle h \rangle_{\rm QCD}$.
The region shaded in orange (blue) is excluded by direct DM searches
(collider searches for the singlet $s$).
Dashed curves show future detection prospects. \label{fig:m_g}
{\bf Right:}
Sample evolution of the DM density, of entropy, of the scalar energy. \label{fig:evo}}
\end{figure}

The DM candidates are the $\SU(2)_X$ vectors with mass $M_X$.
In the usual scenario where they are thermal relics, the
observed DM abundance is reproduced for $g_X^2 \approx M_X/\TeV$~\cite{Hambye:2013sna}
and super-cooling is negligible.
Smaller values of $g_X$ lead to super-cooling, realising the novel DM production mechanism proposed here:
the DM abundance is the sum of the super-cool population, plus the sub-thermal population, Eq.~(\ref{twopopulations}).

We compute the super-cool DM population specializing eq.~\eqref{eq:0.40eV}
and eq.~\eqref{eq:Ysc} to the present model.
We find that the super-cool abundance reproduces the observed DM abundance when
the end of super-cooling is triggered by the QCD phase transition
as $T_{\rm end} = T_{\rm end}^{\rm QCD}$ (eq.~\eqref{eq:endQCD}),
and when reheating is instantaneous.
Thereby $T_{\rm RH} = T_{\rm infl} \approx M_X/8.5$ and the DM abundance simplifies to
\begin{equation}
\Omega_{\rm DM} h^2|_{\rm super-cool}
%\approx 3 \times 10^8 \, \frac{M_X}{\unit{TeV}} \, Y_{\rm DM}|_{\rm super-cool} 
\approx 3.7\times 10^{-3} \, \left( \frac{\langle h \rangle_{\rm QCD}}{\unit[100]{MeV}}\right)^3 \left( \frac{\unit{TeV}}{M_X} \right)^5.
\end{equation}
It does not depend on $g_X$, giving rise to the vertical contours in the $(M_X, g_X)$ plane in the left panel of fig.\fig{m_g}.
%In the opposite limit where the `sub-thermal' contribution dominates, the cosmological DM abundance
%can be reproduced for PeV-scale DM masses, higher than those allowed with freeze-out and
%perturbative couplings.

As anticipated, this is not the end of the story:
one needs to take into account the effects of thermal scatterings after reheating.
One needs to evolve the Boltzmann equation in eq.~\eqref{eq:Bolz} starting from
the initial condition $Y_{\rm DM}(T_{\rm RH}) = Y_{\rm DM}|_{\rm super-cool}$.
The $s$-wave cross-sections for DM annihilations
$VV\leftrightarrow ss$ and  semi-annihilations $VV\leftrightarrow V s$ are~\cite{Hambye:2013sna}
\beq \langle \sigma v\rangle_{\rm ann} =\frac{11g_X^4}{6912\pi M_X^2},\qquad
\langle\sigma v\rangle_{\rm semi-ann} = \frac{g_X^4}{128\pi M_X^2}.
\eeq
In the extreme case where the reheating temperature is larger than the DM decoupling temperature, the 
super-cool population is erased and substituted by the usual thermal relic population.
Otherwise, the super-cool population is negligibly suppressed, and complemented by the additional sub-thermal population
of eq.\eq{YDMthermal}.
For instantaneous reheating ($z_{\rm RH}\approx 8.4$) this evaluates to
$\Omega_{\rm DM} h^2|_{\rm sub-thermal}\approx 0.110 (g_X/0.00020)^4$,
giving rise to the horizontal part of the contour at $g_X \approx 10^{-4}$ in the  $(M_X, g_X)$ plane of fig.\fig{m_g}.
At larger $M_X$ reheating is no longer instantaneous, giving rise to the oblique part of the contour in
fig.~\ref{fig:m_g}a, which shows the complete numerical results for the DM density. Finally, for even larger masses $M_X \gtrsim \unit[300]{TeV}$ the super-cool abundance reproduces the observed DM relic density with $g_X \sim O(1)$, so that super-cooling is ended by nucleation, leading to a DM abundance that depends mainly on $g_X$ and not on $M_X$. Therefore, DM masses can be even PeV-scale or larger, higher than those allowed with freeze-out and perturbative couplings. At $M_X \approx \unit[100]{TeV}$ one has $M_s \simeq M_h$, so that a resonance-like feature in the mixing angle $\alpha$, and consequently in $T_{RH}$ and $\Omega_{DM}$, appears.


In the  region of the parameter space relevant for the present work,
the Spin-Independent cross section for DM direct detection
is dominantly mediated by 
$s$ and simplifies to
\beq \sigma_{\rm SI} = \frac{m_N^4  f^2 }{16\pi v^2}
 \bigg(\frac{1}{m_s^2} - \frac{1}{m_h^2}\bigg)^2 g_X^2 \sin^2 2\alpha
% \simeq \frac{f^2 g_X^2 m_N^4 }{4 \pi M_s^4 w^2} 
 \simeq  \frac{64\pi^3 f^2  m_N^4}{81 M_X^6}\approx
 0.6~10^{-45}\cm^2  (\frac{\TeV}{M_X})^6
\eeq
where $f\approx 0.295$ is the nucleon matrix element and $m_N$ is the nucleon mass. 
So $\sigma_{\rm SI} < 1.5~10^{-45}\cm^2 (M_X/\TeV)$~\cite{1705.06655} for
$M_X > 0.88\TeV $.

%This population is not depleted by (semi)annihilations. To see this, notice that so that the rate of depletion of this super-cool population is
%\begin{equation}
%Y_{\rm DM}|_{\rm super-cool} \, s(T_{RH}) \, \langle \sigma v \rangle \simeq \unit[1.92 \times 10^{-15}]{GeV}\, \left( \frac{\langle h \rangle_{QCD}}{\unit[100]{MeV}}\right)^3 \left( \frac{\unit{TeV}}{M_X} \right)^5  g_X^4
%\end{equation}
%which is much smaller than the Hubble rate $H(T_{\rm RH}) \simeq T_{\rm RH}^2/(0.7 \times \unit[10^{18}]{GeV})$ for 
%\begin{equation}
%0.1 \left( \frac{\langle h \rangle_{QCD}}{\unit[100]{MeV}}\right)^3 \left( \frac{\unit{TeV}}{M_X} \right)^7  g_X^4 \lessapprox 1
%\end{equation}
%which is realized in the parameter region of interest.

% In addition to this first population, a second one can be produced after the end of the period of late-time inflation, starting at $T_{\rm RH}$, by means of inverse annihilations. To estimate when this will happen, by defining $n_{\rm DM} \equiv Y_{\rm DM}|_{\rm super-cool} \, s(T_{RH})$, we may compare the production term $n_{\rm eq}^2(T_{\rm RH}) \langle\sigma v \rangle_{ann}$ with the expansion one $H(T_{\rm RH}) \, n_{\rm DM}$. Therefore, since for the parameters of interest the end of supercooling is triggered by QCD, we find that the production of this second population starts when
%\begin{align}
%\frac{n_{\rm eq}^2(T_{\rm RH}) \langle\sigma v \rangle_{ann}}{H(T_{\rm RH}) \, n_{\rm DM}} \simeq 2.4 \times 10^{22} \left( \frac{\unit[100]{MeV}}{\langle h \rangle_{\rm QCD}}\right)^3 \left( \frac{M_X}{\unit{TeV}}\right)^5  \,\, \left(\frac{M_X}{T_{RH}}\right)^3 \,  g_X^4 \, e^{-2 \frac{M_X}{T_{\rm RH}}}
%\end{align}
%becomes order 1. For $M_X \simeq \unit[500]{GeV}$ and instantaneous reheating this happens for $g_X \gtrsim 10^{-4}$. For larger values of $M_X$ and $g_X$ this happens when the reheating temperature is suppressed as compared to the case of instantaneous reheating.
%
%This second population, produced after the late-time inflation, does not reach thermalization and thus can match the observed relic density. The production rate drops below the Hubble one shortly after $T_{\rm RH}$ (see, for instance, Fig.~\ref{fig:evo}). This is much before the WIMP value $M_X/T \approx 25$, because here the population is much sub-thermal. 

%\footnote{An analytic estimate for the second population, produced after the late-time inflation, can be obtained as follows. In the non-relativistic limit, the Boltzmann equation for the total DM abundance is
%\beq  \frac{dY}{dz} = \frac{\lambda}{z^2} (Y^2 - Y^2_{\rm eq}),\qquad\hbox{where}\qquad
% \lambda =
%{M_{\rm Pl} M \langle\sigma v\rangle}\sqrt{\frac{\pi g_{\rm SM}}{45}}  .
%\label{eq:Boltzf}\eeq
%If $\lambda \gg 1$ freeze-out occurs at $z_{\rm dec} \approx \ln\lambda$; otherwise DM was
%never in thermal equilibrium.
%The  DM population regenerated starting from
%$Y(z_{\rm RH})=0$ at $z_{\rm RH}> z_{\rm dec}$ is
%\beq Y = \lambda \int_{z_{\rm RH}}^\infty \frac{dz}{z^2} Y_{\rm eq}^2 = \lambda \frac{2025g_{\rm DM}^2}{128\pi^7 g_{\rm SM}^2}
%e^{-2z_{\rm RH}} (1+2 z_{\rm RH})\eeq
%Semi-annihilations give an extra suppressed contribution.}

Fig.~\ref{fig:m_g}a  also shows the existing bounds and future discovery prospects, coming both from searches of dark matter via direct detection, and from collider searches for $s$.
The region shaded in orange is excluded by direct searches at XENON1T~\cite{1705.06655} and the dashed vertical lines denote the future sensitivity of XENONnT~\cite{1512.07501}, LZ~\cite{1509.02910} and DARWIN~\cite{1606.07001}.
The direct detection cross section is suppressed by two powers  of the small $g_X$ coupling
and enhanced by the exchange of the 
$s$ scalar state, which is light, see fig.~\ref{fig:infl}b.
As a result the direct detection constraint is significant.
The region shaded in blue is excluded by collider searches for $s$:
the dominant collider bounds come from $s \to e e, \mu \mu$ at CHARM and $B \to K^* \mu \mu$ at LHCb,
as summarized in~\cite{SHiP-NOTE}.
The dashed blue curves indicates the future sensitivity of SHiP~\cite{Anelli:2015pba,SHiP-NOTE}. %\DT{Other relevant future prospects? (Mathusla?)}

\medskip

Finally,  fig.~\ref{fig:m_g}b shows a sample example of the evolution of the DM density,
of entropy, of the energy density in scalars:
the latter dominate during super-cooling, while $n_{\rm DM}$ and $s$ decrease equally.
At reheating almost all of this energy is transferred to entropy, and only a small fraction goes to massive DM.

\subsection{1809.01198 (CSI) - Strong gravitational radiation from a simple dark matter model (Baldes \& Garcia-Cely)}

\subsubsection{Relic density}

\begin{figure}[t]
\begin{center}
\includegraphics[width=440pt]{spin1.pdf}
\end{center}
\caption{The dominant DM annihilation channels for $m_{A} \gg m_{h_D}$ and $\theta \ll 1$.}
\label{fig:freezeout}
\end{figure}

We will consider two production regimes for the DM relic density: the standard freeze-out scenario and super-cool DM.\footnote{Other production mechanism for this model have been discussed in~\cite{Bernal:2015ova}.} The latter only takes place for the classically scale invariant case, i.e. when the gauge symmetry is broken radiatively. Details are given in section \ref{sec:scaleinv}. For the former case, we make the mild assumption that $\lambda_{3}$ and $g_{D}$ are large enough so that DM was in thermal equilibrium with the SM fields in the Early Universe. Freeze-out leads to the observed dark matter abundance, $\Omega h^2 \simeq 0.12$, when the corresponding cross section is of the order $\unit[2.3 \times 10^{-26}]{cm^3/s}$. This means that for given $m_A$, $m_{h_D}$, and $\theta$, the relic density fixes the dark coupling $g_D$. We are interested in the regime in which $m_A > 2m_{h_D}$ so that DM (semi-)annihilates into dark Higgs bosons. We make the further simplifying assumption, $m_{A} \gg m_{h_D}$ and $\theta \ll 1$, so that the annihilations into SM particles by means of a scalar exchange in the s-channel are negligible and the dominant  annihilation channels are those shown in Fig.~\ref{fig:freezeout}. In this regime the correct relic density is achieved for,
	\begin{equation}
	\label{eq:relic}
	g_{D} \approx 0.9 \times \sqrt{\frac{m_{A}}{1 \; \mathrm{TeV}} }\hspace{10pt} \text{and} \hspace{10pt}v_\eta \approx \unit[2.2]{TeV} \times \sqrt{\frac{m_{A}}{1 \; \mathrm{TeV}} }.
	\end{equation}
A more accurate determination can be achieved by numerically solving the Boltzmann equations. Given the uncertainties of the gravitational wave spectrum, however, the use of Eq.~(\ref{eq:relic}) is sufficient for our purposes. The coupling $g_{D}$ is fixed by the relic abundance, which effectively collapses the higher dimensional parameter space to three (one) dimensions in the standard (classically scale invariant) case, which would otherwise have to be scanned over.

\subsubsection{Direct detection}



\begin{figure}[t]
\begin{center}
\includegraphics[width=210pt]{DDplot1.pdf}
\includegraphics[width=210pt]{DDplot2.pdf}
\end{center}
\caption{Mixing angles excluded by Xenon1T~\cite{Aprile:2017iyp} (shaded area)  together with the projected sensitivity from LZ~\cite{Mount:2017qzi} (solid line). Here we assume $m_A\gtrsim \unit[0.1]{TeV}$. \emph{Left:} assuming the relic density is produced via the freeze-out mechanism. \emph{Right:} for the classically scale invariant potential, including contours for some choices of the DM mass.}
\label{fig:DD}
\end{figure}


The spin independent scattering cross-section of dark matter off nucleons is~\cite{Hambye:2008bq}
\begin{equation}
\sigma_{\rm SI} =
\frac{ g_{D}^{4} \, f^{2}  \, m_{N}^{4}  \, v_{\eta}^{2}   }{ 64 \pi \, (m_{N} + m_{A} )^{2} \, v_{\phi}^{2}  } \left( \frac{1}{m_{h}^{2}} - \frac{1}{m_{h_{D}}^{2}}\right)^{2} \, \sin^{2}{2\theta}, 
\label{DirectDetectionEq}
\end{equation}
where $m_N$ denotes the nucleon mass and $f \simeq 0.3$ is a constant that depends on the nucleon matrix element. Thus, current experiments such as Xenon1T~\cite{Aprile:2017iyp,Cui:2017nnn,Akerib:2016vxi} constrain the mixing angle between the scalars. This is shown in Fig.~\ref{fig:DD} assuming $m_A \gtrsim \unit[0.1]{TeV}$ together with the corresponding future sensitivity from LUX-Zepelin~\cite{Aprile:2015uzo,Akerib:2015cja,Mount:2017qzi,Aalbers:2016jon}. In the left panel, the gauge coupling is fixed by freeze out. In the right panel, we consider radiatively-induced symmetry breaking and therefore we use Eq.~\eqref{eq:RISB} to calculate the cross section. No production mechanism is assumed in the latter case.
 
The left panel of the figure can be understood as follows. Working in the limit $m_{A} \gg m_{h_{D}} \gg m_{h}$ and substituting Eq.~(\ref{eq:relic}) into $\sigma_{\rm SI}$, one finds $\sigma_{\rm SI} \propto m_{A} \sin^{2}{2\theta}$, i.e.~with no further dependence on the other DM parameters. Then comparing to direct detection constraints --- which also scale as $\sigma_{\rm SI}^{\rm limit} \propto m_{\rm DM}$ for  $m_{\rm DM} \gtrsim 100$ GeV --- we find current experiments such as Xenon1T demand $\theta \lesssim \mathcal{O}(0.1)$. Future experiments such as LUX-Zepelin, will improve $\sigma_{\rm SI}^{\rm limit}$ by two orders of magnitude and therefore probe down to $\theta \sim \mathcal{O}(0.01)$.
On the other panel, Eq.~\eqref{eq:RISB} indicates that $\sigma_{\rm SI} \propto 1/m_{A}^6 $ with no further dependence on the other dark sector parameters. Hence, $\sigma_{\rm SI}^{\rm limit} \propto m_{\rm DM}$ excludes contours of constant DM mass.  In fact, for the classically invariant case, the  current direct detection constraint demands $m_{A} \gtrsim 0.9$ TeV~\cite{Hambye:2018qjv}.

\subsection{2006.07313 (CSI) - Gravitational wave signals of dark matter freeze-out (Marfatia \& Cheng)}

\subsubsection{Dark matter abundance}


Having calculated $T_{\rm infl}$, $T_{\rm end}$
and $T_{\rm rh}$, we now consider the DM relic abundance in two regimes: 
$T_{\rm rh}> T_{\rm dec}$ and $T_{\rm rh}< T_{\rm dec}$,
where $T_{\rm dec}$ is the decoupling temperature in the conventional freeze-out scenario.
For $T_{\rm rh} < T_{\rm dec}$, the DM abundance is dictated by  
supercooling and by sub-thermal production via scattering.
Although we account for bubble filtering, its effect is negligible.
On the other hand, for $T_{\rm rh}> T_{\rm dec}$, the
supercooled population is washed out, and the sub-thermal population reattains thermal
equilibrium and produces the relic abundance as in the standard freeze-out scenario. 
The $\Omega_{\rm DM}h^2=0.11$ contour in the upper-left corner of Fig.~\ref{fig:su2x_Oh2} corresponds to this case.








The DM abundance resulting from inflationary supercooling is 
\begin{eqnarray}
\frac{n_{\rm DM}|_{T=T_{\rm rh}}}{s|_{T=T_{\rm rh}}}= \frac{45 g_{\rm DM}}{2\pi^4 g_*}\frac{T_{\rm rh}}{T_{\rm infl}} \left( \frac{T_{\rm end}}{T_{\rm infl}} \right)^3
\times f_{\rm in}\,,
%~~~~~~
%Y^{\rm eq}_{\rm DM}= \frac{45 g_{\rm DM}}{2\pi^4 g_*}\,,
\end{eqnarray}
where $f_{\rm in} \equiv (n^{\rm in}_\chi|_{T_{\rm end}})
/(n^{\rm eq}_\chi|_{T_{\rm end}})$ quantifies the filtering effect with $T_\star = T_{\rm end}$ in Eq.~(\ref{eq:filter_analytic}).
%
However, $f_{\rm in} =1$ for most of the parameter space of this model
because the bubble wall velocity 
is close to the speed of light
and $\gamma_w T_{\rm end} \gg m_{\chi}$.
%
The dilution from supercooling is significant 
for $T_{\rm infl}/T_{\rm end} \gg 1$, and can lead to DM being under-produced;
this corresponds to the white region in the lower-right corner 
of Fig.~\ref{fig:su2x_Oh2}.
%
The DM density today can be calculated by rescaling from $T_{\rm rh}$ to the temperature today, 0.235~meV, and using Eq.~(\ref{eq:rescale}).

\begin{figure}[t]
\centering
\includegraphics[height=3.8in,angle=270]{mx_gx_Oh2.pdf}
\caption{\small \label{fig:su2x_Oh2}
 $\Omega_{\rm DM}h^2$ for the $SU(2)_X$ Model with $\langle h \rangle_{\rm QCD}=100~{\rm MeV}$.
The black-dashed contours indicate the observed DM relic abundance, $\Omega_{\rm DM}h^2=0.11$.
The stars mark the six benchmark points in Table~\ref{tab:su2x_BP}.
}
\end{figure}

We now consider sub-thermal DM production after supercooling. The decoupling temperature
of this population is $T_{\rm dec}\simeq m_\chi/\ln \lambda$, where 
$\lambda\equiv M_{\rm pl}m_\chi \langle \sigma_{\rm ann}v \rangle \sqrt{\pi g_\star/45}$, and
$\langle \sigma_{\rm ann}v \rangle$ is the thermal averaged DM annihilation cross section 
of the ${\rm DM}{\rm DM} \to \eta \eta$ 
process~\cite{Hambye:2018qjv}.
The abundance of the sub-thermal population is obtained by solving the Boltzmann equation.
%

For $T_{\rm rh} < T_{\rm dec}$, both supercooling and sub-thermal production contribute to the DM relic abundance,
\begin{eqnarray}
\Omega_{\rm DM}h^2=\Omega_{\rm DM}h^2|_{\rm supercool}
+\Omega_{\rm DM}h^2|_{\rm sub-thermal}\,.
\end{eqnarray}
For $T_{\rm rh} > T_{\rm dec}$, the plasma thermalizes again,  and the usual freeze-out mechanism yields the relic abundance,
\begin{eqnarray}
\Omega_{\rm DM}h^2=\Omega_{\rm DM}h^2|_{\rm freeze-out}\simeq
0.11 \times \frac{\langle \sigma_{\rm ann}v \rangle}{2\times 10^{-26}~{\rm cm^3/s}}\,.
\end{eqnarray}
%
The DM relic abundance
is shown in Fig.~\ref{fig:su2x_Oh2}.
We mark six benchmark points along the dashed curves (which indicate $\Omega_{\rm DM}h^2\simeq 
0.11$), 
and their values are listed in Table~\ref{tab:su2x_BP}.
%
For {\bf BP2} and {\bf BP3} sub-thermal processes dominate.
Dilution by supercooling fixes the DM abundances for 
{\bf BP1}, {\bf BP4}, {\bf BP5}, and {\bf BP6}.
%
The end of supercooling occurs at the nucleation temperature for  {\bf BP4}, {\bf BP5} and {\bf BP6}, and at the QCD phase transition temperature for {\bf BP1}.
%
 For the $\Omega_{\rm DM}h^2=0.11$ contour in the upper-left corner of Fig.~\ref{fig:su2x_Oh2}, $T_{\rm rh} > T_{\rm dec}$
 and the DM abundance is produced by the usual thermal freeze-out.
However, we have checked that the pressure difference due to transition radiation across the wall  becomes larger than the 
vacuum pressure driving the bubble expansion~\cite{Bodeker:2017cim}. Since this renders our assumption that
GWs are predominately produced by bubble collisions invalid, we do not consider this part of the parameter space any further.




\begin{table}[H]
\caption{\small \label{tab:su2x_BP}
Benchmark points for the $SU(2)_X$ Model that give $\Omega_{\rm DM}h^2=0.11$. 
Note that $T_\star=T_{\rm infl}$.
}
%\begin{ruledtabular}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{c|cccccc}
\hline
\hline
    & {\bf BP1} & {\bf BP2} & {\bf BP3} & {\bf BP4} 
    & {\bf BP5} & {\bf BP6} \\
\hline
$m_\chi/{\rm GeV}$  & 540 & $5.4\times 10^3$ 
                    & $4.2\times 10^4$ & $3.0\times 10^5$ 
                    &  $8\times 10^7$   & $6\times 10^9$   \\
$g_X$               & $1.7\times 10^{-5}$ & $1.5\times 10^{-3}$ 
                    & $5.9\times 10^{-2}$ & $0.72$ 
                    &  $0.77$  & $0.82$  \\
\hline
$\alpha$  & $1.3\times 10^{14}$ & $1.2\times 10^{22}$ 
          & $1.8\times 10^{29}$ & $4.4\times 10^{16}$ 
          & $2.8\times 10^{13}$ & $9.4\times 10^{10}$  \\
$\beta/H_\star$ & $3.5\times 10^{11}$ & $8.1\times 10^6$ 
                & $1.3\times 10^3$ & 10.7 
                & 12.5 & 14.4  \\
$v_\eta/T_{\rm end}$ & $3.4\times 10^9$ & $3.7\times 10^9$ 
                     & $6.0\times 10^9$ & $3.4\times 10^{5}$ 
                     & $5.1\times 10^4$ & $1.2\times 10^4$  \\
$\gamma_w$ & $2.9\times 10^5$ & $2.9\times 10^7$ 
           & $1.8\times 10^9$ & $1.2\times 10^6$ 
           & $2.0\times 10^5$ & $4.7\times 10^4$  \\
$T_{\rm end}/{\rm GeV}$ & $1.85\times 10^{-2}$ & $1.87 \times 10^{-3}$ 
                    & $2.4\times 10^{-4}$ & 2.42 
                    & $4.01\times 10^3$ & $1.27\times 10^6$  \\
$T_{\rm rh}/{\rm GeV}$ & 46.6 & 422 
                       & 2082 & 3566 
                       & 14.5 & 0.201  \\
$T_{\rm infl}/{\rm GeV}$ & 63.6 & 629 
                    & $4.95\times 10^{3}$ & $3.53\times 10^{4}$ 
                    & $9.29\times 10^6$ & $7.08\times 10^8$  \\
%
\hline
\hline
\end{tabular}
%\end{ruledtabular}
\end{adjustbox}
\end{table}

\subsection{2105.14387}

\subsection{Summary of results}

%Wikipedia: The cuspy halo problem (also known as the core-cusp problem) refers to a discrepancy between the inferred dark matter density profiles of low-mass galaxies and the density profiles predicted by cosmological N-body simulations. Nearly all simulations form dark matter halos which have "cuspy" dark matter distributions, with density increasing steeply at small radii, while the rotation curves of most observed dwarf galaxies suggest that they have flat central dark matter density profiles ("cores").

%1404.5313: Measurements of the stellar velocity dispersions, indicate systematically lowercentral mass estimates than simulations predict for large subhalos – that is, the Milky Way dwarf spheroidal galaxies are systematically less dense than the subhalos expected to host them, a problem that has been dubbed “Too Big to Fail” (TBTF). 
%While possibly related to the missing satellites problem, in that the largest subhalos may not have been found, TBTF is a distinct problem related to the internal structure of subhalos, rather than strictly their abundances.


\appendix
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\section{Running couplings, thermal masses}
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\subsection{RGEs}
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

For scalar self-couplings $\lambda_H$ and $\lambda_\phi$, and the portal coupling $\lambda_{\rm P}$ we have:
\begin{eqnarray}
&&(4\pi)^2 \frac{\dd \lambda_H}{\dd \ln \mu}=-6 y_t^4+24\lambda_H^2+2\lambda_{\rm P}^2 +
\lambda_H \left(12y_t^2-\frac{9}{5}g_1^2-9g_2^2\right) +\frac{27}{200}g_1^4+\frac{9}{20}g_2^2g_1^2
+\frac{9}{8}g_2^4\qquad \quad
\label{lHeqn}
% \nonumber\\ 
\\
&&(4\pi)^2 \frac{\dd \lambda_\phi}{\dd \ln \mu}= 24\lambda_\phi^2 +2\lambda_{\rm P}^2
-9\lambda_\phi \, g_{\mathrm{X}}^2 +\frac{9}{8} g_{\mathrm{X}}^4\\ 
&&(4\pi)^2 \frac{\dd \lambda_{\rm P}}{\dd \log \mu}=\lambda_{\rm P}\left(6y_t^2
+12\lambda_H+12\lambda_\phi
-4\lambda_{\rm P}
-\frac{9}{2}g_{\mathrm{X}}^2-\frac{9}{10}g_1^2-\frac{9}{2}g_2^2\right)\,,
\end{eqnarray}
where the top Yukawa coupling obeys
\begin{eqnarray}
(4\pi)^2 \frac{\dd y_t}{\dd \ln \mu}=y_t\left(\frac{9}{2}y_t^2 -\frac{17}{20}g_1^2-\frac{9}{4}g_2^2-8g_3^2\right)\,,
\end{eqnarray}
and $g_{\mathrm{X}}$, $g_{3,2,1}$ are the gauge couplings of the SU(2)$_{\mathrm{X}} \times$ SU(3) $\times$ SU(2) $\times$ U(1),
\begin{eqnarray}
&&(4\pi)^2 \frac{\dd g_{\mathrm{X}}}{\dd \ln \mu}=-\frac{43}{6}g_{\mathrm{X}}^3-\frac{1}{(4\pi)^2}\frac{259}{6}g_{\sst \mathrm{CW}}^5\\
\nonumber\\
&&(4\pi)^2 \frac{\dd g_3}{\dd \log \mu}=-7g_3^3 \,,\quad
(4\pi)^2 \frac{\dd g_2}{\dd \log \mu}=-\frac{19}{6}g_2^3  \,,\quad
(4\pi)^2 \frac{\dd g_1}{\dd \log \mu}=\frac{41}{10}g_1^3\,,
\end{eqnarray}
where for the U(1) coupling we use the 
normalisation $g_1^2 = \frac{5}{3} g_Y^2$.

%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\subsection{Thermal masses}
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
The thermal corrections to the mass matrix of the two scalars are given at leading order in the high-temperature expansion by
\begin{align}
\begin{pmatrix}
m_{hh,T}^2 & m_{h \varphi, T}^2 \\ m_{\varphi h,T}^2 & m_{\varphi \varphi,T}^2
\end{pmatrix} = &\begin{pmatrix}
m_{hh}^2 & m_{h \varphi}^2 \\ m_{\varphi h}^2 & m_{\varphi \varphi}^2
\end{pmatrix} \notag \\ &+
\begin{pmatrix}
\qty(\frac{1}{4}\lambda_1 + \frac{1}{24} \lambda_2 + \frac{3}{16} g^2 + \frac{1}{16} g'^2+\frac{1}{4} y_t^2)T^2 & 0 \\
0 & \qty(\frac{1}{4}\lambda_3 + \frac{1}{24} \lambda_2 + \frac{3}{16} g_x^2 )T^2
\end{pmatrix}.
\end{align}
The thermal masses of the two scalars are obtained by diagonalising this matrix. The factors of the scalar couplings differ from the results of other literature (e.g. ref. \cite{Carrington:1992}) since we did not include the effect of the Goldstone bosons in our computations.

At leading order in the high-temperature expansion only the longitudinal gauge bosons acquire a thermal mass. In the gauge field basis ($A_\mu^a$ and $B_\mu$) before electroweak symmetry breaking the longitudinal thermal masses read~\cite{Carrington:1992, Sannino:2015}
\begin{align}
M_L^2(h,T) = \frac{h^2}{4} \begin{pmatrix}
g^2 && 0 && 0 && 0 \\ 0 && g^2 && 0 && 0 \\ 0 && 0 && g^2 && - g g' \\  0 && 0 && -g g' && g'^2
\end{pmatrix} +\frac{11}{6} T^2 \begin{pmatrix}
g^2 && 0 && 0 && 0 \\ 0 && g^2 && 0 && 0 \\ 0 && 0 && g^2 && 0 \\  0 && 0 && 0 && g'^2
\end{pmatrix}.
\end{align}
Transforming the above matrix to the $W_\mu^+$, $W_\mu^-$, $Z_\mu$ and $A_\mu$ basis, we obtain the thermal masses of the longitudinal $W$, $Z$ and photon \cite{Rose:2015}
\begin{align}
M^2_{W_L} &= m_W^2(h) + \frac{11}{6} g^2 T^2, \label{eq:thermal-mass-first}\\
M^2_{Z_L} &= \frac{1}{2} m_Z^2(h) +\frac{11}{12} \frac{g^2}{\cos^2(\theta_W)} T^2 + \frac{\Delta}{2},\\
M^2_{\gamma_L} &=\frac{1}{2} m_Z^2(h)+  \frac{11}{12} \frac{g^2}{\cos^2(\theta_W)} T^2 - \frac{\Delta}{2}, \\
\Delta^2 &= m_Z^4(h) + \frac{11}{3} \frac{g^2 \cos^2(2\theta_W)}{\cos^2(\theta_W)}\qty[m_Z^2(h) + \frac{11}{12} \frac{g^2}{\cos^2(\theta_W)} T^2] T^2.\label{eq:thermal-mass-last}
\end{align}
\par
For the gauge bosons of the hidden gauge group, the thermal masses resemble the ones for the $W$ bosons but with the gauge coupling $g_X$. However, the factor $11/6$ is replaced by $5/6$ since the $X$ gauge boson does not couple to any fermions,
\begin{align}
M_{X_L}^2 =  m_X^2(\varphi) + \frac{5}{6} g_X^2 T^2 .
\label{xthermal}
\end{align}

%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\section{Review of the literature}
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

\begin{description}
\item[Hambye-Teresi-Strumia~\cite{Hambye:2018}]
\begin{itemize}
\item thermal evolution: super-cooling, possibility of QCD-induced end of the phase transition, results for the nucleation temperature, reheating temperature and number of e-folds of thermal inflation.
\item reheating: compute the rate $\Gamma$ at which the scalar energy is dissipated solving the scalar equations of motion and assuming that $\Gamma=\Gamma_h \sin^2 \alpha+\Gamma_s \cos^2 \alpha$, where $\alpha$ is the mixing angle between the scalars (in their convention). They claim that the reheating temperature is close to the temperature before inflation if the gauge coupling is sufficiently large. Results for the reheating temperature in the $(M_X, g_X)$ plane.
\item DM production: super-cooling + thermal freeze-out
\item DM direct detection
\item assume that the new scalar is much lighter than the Higgs (see the top of page 7 and figure~2 --- $M_S<10\g$, however, in fig. 3 Teresi claimed to have included the scenario with the scalar being heavier than the Higgs)
\item resonant leptogenesis + Higgs decays; Boltzmann equations solved for a single-flavour approximation for the SM leptons.
\end{itemize}
\item[Baldes-Garcia Cely~\cite{Baldes:2018}]
\begin{itemize}
\item thermal evolution: ``sequential symmetry breaking'' --- first a VEV for the new scalar, then for the Higgs (1-field effective potential used); possibility of QCD-induced phase transition
\item DM production: freeze-out + super-cooling (although they are aware of other mechanisms, citing ref.~\cite{Bernal:2015}, they do not discuss whether other mechanisms are subdominant); assume $M_X\gg M_S$
\item DM direct detection
\item gravitational waves: show where Bodeker-Moore bound is satisfied, estimate signal to noise ratio, use sound waves (comment that if a lot of inflation is present, the scalar contribution might be more  important), take into account the reheating temperature
\end{itemize}
\item[Khoze et al~\cite{Khoze:2013-2, Plascencia:2016}]
\begin{itemize}
\item ARS leptogenesis, no scalar decays
\item it is assumed that the critical temperature is of the same order as the nucleation temperature and as the vev of the new scalar field, while these are orders of magnitude apart
\end{itemize}
\end{description}


%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\section{Dark matter details}
%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

\subsection{$2 \rightarrow 2$ cross sections}

arXiv: 1406.4104

There are six contributions to the annihilation cross-section: the first one has two $h_1$ particles in the final state, the third one has two $h_2$ particles, while the second one has one of each scalar. The last three contributions are related respectively to the production of a couple of W, a couple of Z or a couple of top quarks.


\begin{align}
\begin{split}
\sigma v_{\text{ann}}^{h_1,h_1}&=\frac{g_X^2}{110592 \pi  M_X^3} \sqrt{M_X^2-M_{h_2}^2}\\
&\times\left(\frac{16 g_X^2 \cos ^4\alpha \left(11 M_{h_2}^4-28 M_{h_2}^2 M_X^2+44 M_X^4\right)}{\left(M_{h_2}^2-2 M_X^2\right)^2}\right.\\
&+\frac{8 g_X M_X \cos ^2\alpha \left(M_{h_2}^2-10 M_X^2\right) \mathcal{A}_1 }{\left(4 M_X^2-M_{h_1}^2\right) \left(M_{h_2}^2-4 M_X^2\right) \left(M_{h_2}^2-2 M_X^2\right)}\\
&\left.+\frac{3 M_X^2 \mathcal{A}_1^2}{\left(M_{h_1}^2-4 M_X^2\right)^2 \left(M_{h_2}^2-4 M_X^2\right)^2}\right)
\end{split}
\end{align}

\begin{align}
\begin{split}
\mathcal{A}_1&=w (\lambda_{HS}-6\lambda_S) \left(3 M_{h_1}^2+M_{h_2}^2-16 M_X^2\right)\\
&+2 v \sin (2 \alpha ) \left(M_{h_1}^2 (6\lambda_H-3\lambda_{HS})-M_{h_2}^2 (6\lambda_H+\lambda_{HS})+16\lambda_{HS} M_X^2\right)\\
&-4 w \cos (2 \alpha ) \left(6\lambda_S M_{h_1}^2+\lambda_{HS} M_{h_2}^2-4 M_X^2 (\lambda_{HS}+6\lambda_S)\right)\\
&-3 v \sin (4 \alpha ) (2\lambda_H+\lambda_{HS}) \left(M_{h_1}^2-M_{h_2}^2\right)\\
&-3 w \cos (4 \alpha ) (\lambda_{HS}+2\lambda_S) \left(M_{h_1}^2-M_{h_2}^2\right)
\end{split}
\end{align}

\begin{align}
\begin{split}
&\sigma v_{\text{ann}}^{h_1,h_2}=\frac{g_X^2}{221184 \pi  M_X^8} \sqrt{M_{h_1}^4-2 M_{h_1}^2 \left(M_{h_2}^2+4 M_X^2\right)+\left(M_{h_2}^2-4 M_X^2\right)^2}\\
&\times\left(\frac{g_X^2 \sin ^2(2 \alpha )}{\left(M_{h_1}^2+M_{h_2}^2-4 M_X^2\right)^2}\right.\\
&\qquad \left(-224 M_X^6 \left(M_{h_1}^2+M_{h_2}^2\right)-12 M_X^2 \left(M_{h_1}^2-M_{h_2}^2\right)^2 \left(M_{h_1}^2+M_{h_2}^2\right)\right.\\
&\left.\qquad+\left(M_{h_1}^2-M_{h_2}^2\right)^4+M_X^4 \left(92 M_{h_1}^4-8 M_{h_1}^2 M_{h_2}^2+92 M_{h_2}^4\right)+704 M_X^8\right)\\
&+\frac{2 g_X M_X^3 \sin (2 \alpha ) \left(M_{h_1}^4+M_{h_2}^4-2 M_{h_1}^2 \left(M_{h_2}^2+M_X^2\right)-2 M_{h_2}^2 M_X^2+40 M_X^4\right) \mathcal{A}_2 }{\left(M_{h_1}^2-4 M_X^2\right) \left(4 M_X^2-M_{h_2}^2\right) \left(M_{h_1}^2+M_{h_2}^2-4 M_X^2\right)}\\
&+\left.\frac{3 M_X^6 \mathcal{A}_2^2}{\left(M_{h_1}^2-4 M_X^2\right)^2 \left(M_{h_2}^2-4 M_X^2\right)^2}\right)
\end{split}
\end{align}

\begin{align}
\begin{split}
\mathcal{A}_2&=v (6 \lambda_H-\lambda_{HS}) \left(M_{h_1}^2-M_{h_2}^2\right)\\
&-4 \lambda_{HS} v \cos (2 \alpha ) \left(M_{h_1}^2+M_{h_2}^2-8 M_X^2\right)\\
&+2 w \sin (2 \alpha ) (\lambda_{HS}+6 \lambda_S) \left(M_{h_1}^2+M_{h_2}^2-8 M_X^2\right)\\
&-3 v \cos (4 \alpha ) (2 \lambda_H+\lambda_{HS}) \left(M_{h_1}^2-M_{h_2}^2\right)\\
&+3 w \sin (4 \alpha ) (\lambda_{HS}+2 \lambda_S) \left(M_{h_1}^2-M_{h_2}^2\right)
\end{split}
\end{align}

\begin{align}
\begin{split}
\sigma v_{\text{ann}}^{h_2,h_2}&=\frac{g_X^2}{110592 \pi  M_X^3} \sqrt{M_X^2-M_{h_1}^2} \\
&\times\left(\frac{16 g_X^2 \sin ^4\alpha \left(11 M_{h_1}^4-28 M_{h_1}^2 M_X^2+44 M_X^4\right)}{\left(M_{h_1}^2-2 M_X^2\right)^2}\right.\\
&-\frac{8 g_X M_X \sin ^2\alpha \left(10 M_X^2-M_{h_1}^2\right)\mathcal{A}_3}{\left(M_{h_1}^2-4 M_X^2\right) \left(M_{h_1}^2-2 M_X^2\right) \left(4 M_X^2-M_{h_2}^2\right)}\\
&+\left.\frac{3 M_X^2 \mathcal{A}_3^2}{\left(M_{h_1}^2-4 M_X^2\right)^2 \left(M_{h_2}^2-4 M_X^2\right)^2}\right)
\end{split}
\end{align}

\begin{align}
\begin{split}
\mathcal{A}_3&=w (\lambda_{HS}-6 \lambda_S) \left(M_{h_1}^2+3 M_{h_2}^2-16 M_X^2\right)\\
&+2 v \sin (2 \alpha ) \left(M_{h_1}^2 (6 \lambda_H+\lambda_{HS})+M_{h_2}^2 (3 \lambda_{HS}-6 \lambda_H)-16 \lambda_{HS} M_X^2\right)\\
&+4 w \cos (2 \alpha ) \left(\lambda_{HS} M_{h_1}^2+6 \lambda_S M_{h_2}^2-4 M_X^2 (\lambda_{HS}+6 \lambda_S)\right)\\
&+3 v \sin (4 \alpha ) (2 \lambda_H+\lambda_{HS}) \left(M_{h_1}^2-M_{h_2}^2\right)\\
&+3 w \cos (4 \alpha ) (\lambda_{HS}+2 \lambda_S) \left(M_{h_1}^2-M_{h_2}^2\right)
\end{split}
\end{align}

\begin{equation}\sigma v_{\text{ann}}^{WW}=\frac{g_X^2 \sin ^2(2 \alpha ) \left(M_{h_1}^2-M_{h_2}^2\right)^2 \left(3 M_W^4-4 M_W^2 M_X^2+4 M_X^4\right) \sqrt{M_X^2-M_W^2}}{288 \pi  M_X v^2 \left(M_{h_1}^2-4 M_X^2\right)^2 \left(M_{h_2}^2-4 M_X^2\right)^2}\end{equation}

\begin{equation}\sigma v_{\text{ann}}^{ZZ}=\frac{g_X^2 \sin ^2(2 \alpha ) \left(M_{h_1}^2-M_{h_2}^2\right)^2 \left(3 M_Z^4-4 M_X^2 M_Z^2+4 M_X^4\right) \sqrt{M_X^2-M_Z^2}}{576 \pi  M_X v^2 \left(M_{h_1}^2-4 M_X^2\right)^2 \left(M_{h_2}^2-4 M_X^2\right)^2}\end{equation}

\begin{equation}\sigma v_{\text{ann}}^{tt}=\frac{g_X^2 \sin ^2(2 \alpha ) M_t^2 \left(M_{h_1}^2-M_{h_2}^2\right)^2 \left(M_t^2-M_X^2\right) \sqrt{M_X^2-M_t^2}}{288 \pi  M_X v^2 \left(M_{h_1}^2-4 M_X^2\right)^2 \left(M_{h_2}^2-4 M_X^2\right)^2}\end{equation}

The semiannihilation cross section is
\begin{align}
\begin{split}\sigma_\text{semiann}v&=\frac{g_X^4 \left(M_{h_1}^4-10 M_{h_1}^2 M_X^2+9 M_X^4\right)^{3/2} \sin^2 (\alpha )}{128 \pi  M_X^4 \left(M_{h_1}^2-3 M_X^2\right)^2}\\
&+\frac{g_X^4 \left(M_{h_2}^4-10 M_{h_2}^2 M_X^2+9 M_X^4\right)^{3/2} \cos^2 (\alpha )}{128 \pi  M_X^4 \left(M_{h_2}^2-3 M_X^2\right)^2}.
\end{split}
\end{align}

1707.01434 for $3 \rightarrow 2$ processes





























